The Responsible Foundation Model Development Cheatsheet: A Review of Tools & Resources

Foundation model development attracts a rapidly expanding body of contributors, scientists, and applications. To help shape responsible development practices, we introduce the Foundation Model Development Cheatsheet: a growing collection of 250+ tools and resources spanning text, vision, and speech modalities. We draw on a large body of prior work to survey resources (e.g. software, documentation, frameworks, guides, and practical tools) that support informed data selection, processing, and understanding, precise and limitation-aware artifact documentation, efficient model training, advance awareness of the environmental impact from training, careful model evaluation of capabilities, risks, and claims, as well as responsible model release, licensing and deployment practices. We hope this curated collection of resources helps guide more responsible development. The process of curating this list, enabled us to review the AI development ecosystem, revealing what tools are critically missing, misused, or over-used in existing practices. We find that (i) tools for data sourcing, model evaluation, and monitoring are critically under-serving ethical and real-world needs, (ii) evaluations for model safety, capabilities, and environmental impact all lack reproducibility and transparency, (iii) text and particularly English-centric analyses continue to dominate over multilingual and multi-modal analyses, and (iv) evaluation of systems, rather than just models, is needed so that capabilities and impact are assessed in context.

==> TMLR/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/00_previous_introduction.tex <==
% \vspace{-6mm}
\section*{A Guide: Resources for Best Development Practices}
\label{sec:guide}

\paragraph{Why?} 
This cheatsheet serves as a succinct guide, prepared \emph{by} foundation model developers \emph{for} foundation model developers.
The intended audience is a range of foundation model developers, including academic researchers, startup companies, research labs, who are pretraining from scratch, or simply finetuning, big and small.
As the field of AI foundation model development rapidly expands, welcoming new contributors, scientists, and applications, we hope to lower the barrier for new community members to become familiar with the variety of resources, tools, and findings.
The focus of this cheatsheet is not only, or even primarily, to support building, but to inculcate good practices, awareness of limitations, and general responsible habits as community norms.
While it is certainly not comprehensive, we have selected a sample of resources that we have found useful and would recommend for consideration by others.
We hope it will serve as a general guide to promote responsible development practices, as well as building new models and infrastructure in our field.
%This document provides contextualized information and a static sample of the cheatsheet---the fully documented, live cheatsheet is available at \url{fmcheatsheet.org}.

% \vspace{-2mm}
\paragraph{What?}
There are many exceedingly popular tools to build, distribute and deploy foundation models.
But there are also many outstanding resources that receive less attention or adoption, in part because of developers' haste to accelerate, deploy, and monetize.
We hope to bring wider attention to these core resources that support \emph{informed} data selection, processing, and understanding (\cref{sec:data,sec:data-prep}), \emph{precise and limitation-aware} artifact documentation (\cref{sec:documentation}), \emph{efficient} model training (\cref{sec:model-training}), \emph{advance awareness} of the environmental impact from training (\cref{sec:environmental-impact}), \emph{careful} model evaluation of capabilities, risks, and claims (\cref{sec:model-eval}), as well as \emph{responsible} model release and deployment practices (\cref{sec:model-release}).

In each section we introduce considerations for that phase of development.
We suggest developers building models from scratch carefully consider their data sources and curation processes to avoid unintended risk (e.g. privacy, copyright, inappropriate content), marginalization (e.g. by accidental filtering), or unexpected model behaviors (e.g. text distribution has unintended quirks). 
Data processing should consider how to deduplicate, filter, decontaminate, and mix different data sources towards the intended distribution and characteristics.
We recommend this process is carefully documented for reproducibility and understanding.
If new data is released, setting its governance standards early will avoid misuse later, and adding structure to documentation will allow for its properties to be easily preserved, understood, and respected in downstream data mixes or compositions.
Model training can be financially and environmentally expensive.
Resources for estimating environmental impact can break down these costs and simplify the considerations.
Newly trained models should be carefully evaluated for their intended uses, as well as foreseeable misuses or harms.
We suggest resources to taxonomize and contextualize evaluations, without over-claiming or misunderstanding the limitations of the reported numbers.
Lastly, we suggest how developers can make an informed selection of licenses, and release mechanisms, to mitigate potential misuses.


% \vspace{-2mm}
\paragraph{Criteria for Inclusion.}
\label{sec:criteria}
The resources are selected based on a literature review for each phase of foundation model development. Inclusion is predicated on a series of considerations, including: the perceived helpfulness as a development tool, the extent and quality of the documentation, the insights brought to the development process, and, in some cases, the lack of awareness a useful resource has received in the AI community.
For an example of this last consideration, in \cref{sec:finetune} we try to include more Finetuning Data Catalogs for lower resource languages, that often receive less attention than HuggingFace's Dataset library.
Rather than sharing primarily academic literature as in a traditional survey work, we focus on tools, such as data catalogs, search/analysis tools, evaluation repositories, and, selectively, literature that summarizes, surveys or guides important development decisions.
As with any survey, these principles for inclusion are incomplete and subjective, but we hope to remedy this with the open call for community contributions.

% \vspace{-2mm}
\paragraph{How to contribute?}
We intend for the web version of the cheatsheet to be a crowdsourced, interactive, living document, with search and filter tools.
To contribute to this resource, follow instructions given in the website.
Contributions should be scoped to resources, such as tools, artifacts, or helpful context papers, that directly inform responsible foundation model development.
Significant contributions will be recognized in the web search tool, and in follow up write-ups to this guide.
Contributed content will be reviewed by authors, to assess that the resources fit the aspirational criteria for inclusion outlined above.

% \vspace{-2mm}
\paragraph{Scope \& Limitations.} 
We've compiled resources, tools, and papers that have helped guide our own intuitions around model development, and which we believe will be especially helpful to nascent (and sometimes even experienced) developers in the field.
However, this guide is far from exhaustive---and here's what to consider when using it:

\begin{itemize} %[itemsep=1pt]%, wide=5pt]
    \item We scope these resources to newer foundation model developers, usually releasing models to the community. Larger organizations, with commercial services, have even broader considerations for responsible development and release.
    \item Foundation model development is a rapidly evolving science. %\textbf{This document is only a sample, dated to January 2024.} The full cheatsheet is more comprehensive and open for on-going public contributions: \url{fmcheatsheet.org}.
    \item We've scoped our data modalities only to \textbf{text, vision, and speech}. 
    We support multilingual resources, but acknowledge this is only a starting point.
    \item A cheatsheet \textbf{cannot be comprehensive}. We prioritize resources we have found helpful, and rely heavily on survey papers and repositories to point out the many other awesome works which deserve consideration, especially for developers who plan to dive deeper into a topic.
    \item \textbf{We cannot take responsibility for these resources---onus is on the reader to assess their viability, particularly for their circumstance.} At times we have provided resources with conflicting advice, as it is helpful to be aware of divided community perspectives. Our notes throughout are designed to contextualize these resources, to help guide the reader's judgement.
\end{itemize}

% \vspace{-2mm}
\paragraph{Notations and Symbols}
This cheatsheet provides tables for several topics, with symbols for brevity.
Modalities are indicated for text ~\TextCircle[0.75]{}, vision~\VisionCircle[0.75]{}, and speech ~\SpeechCircle[0.75].
We also provide hyperlinks for ArXiv \earxiv[1.2em][-0.4ex]\hspace{0.25em}, for Hugging Face objects \ehf[1.2em][-0.4ex]\hspace{0.25em}, for GitHub \egithub[1.2em][-0.4ex]\hspace{0.25em}, and for webpages \eweb[1.2em][-0.4ex]\hspace{0.25em}.

% \vspace{-2mm}
\paragraph{Who are we?}
An organic collective of volunteers have contributed to this cheatsheet, spanning developers of several notable datasets (MasakhaNER \citep{adelani2021masakhaner}, the Pile \citep{gao2020pile}, ROOTS \citep{NEURIPS2022_ce9e92e3}, Dolma \citep{dolma}, the Flan Collection \citep{longpre2023flan}, the Data Provenance Collection \citep{longpre2023data}), models (OpenFlamingo \citep{awadalla2023openflamingo}, Pythia \citep{biderman2023pythia}, Flan-PaLM \citep{chung2022scaling}, RWKV \citep{peng2023rwkv}), and benchmarks (LM Eval Harness \citep{eval-harness}, HELM \citep{liang2022holistic}) in the community.
Most importantly, contributors (\cref{app:contributions}) have carefully assembled the tools and resources that have enabled them to build this infrastructure responsibly with an eye on social and scientific impact.

\begin{figure*}[ht]
    \centering
    \begin{subfigure}{0.94\textwidth}
        \includegraphics[width=\textwidth]{logos/cheatsheet-flow.pdf}
    \end{subfigure}
    % \caption{\textbf{} }
    \label{fig:cheatsheet-flow}
    \vspace{-3mm}
\end{figure*}

\input{tables/review}

==> tables/code-reproducibility-1.tex <==
\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 
\midrule

    \multicolumn{4}{c}{\textsc{\emph{Code Reproducibility}}} \\
    \midrule

\TextCircle\VisionCircle\SpeechCircle & \textbf{Anaconda} & An environment and dependency management tool. & \emojiblank\emojiblank\emojiblank\href{https://www.anaconda.com/}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Colab Notebooks} & A tool to execute and share reproducible code snippets. & \emojiblank\emojiblank\emojiblank\href{https://colab.research.google.com/}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Docker} & An environment and dependency management tool. & \emojiblank\emojiblank\emojiblank\href{https://docker-curriculum.com/}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Jupyter Notebooks} & A tool to execute and share reproducible code snippets. & \emojiblank\emojiblank\emojiblank\href{https://jupyter.org/}{\eweb} \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{LM Evaluation Harness} & Orchestration framework for standardizing LM prompted evaluation, supporting hundreds of subtasks \citep{eval-harness}. & \emojiblank\emojiblank\href{https://github.com/EleutherAI/lm-evaluation-harness}{\egithub}\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Semver} & A widely used protcol for versioning to software, to ensure easy reproducibility. & \emojiblank\emojiblank\emojiblank\href{https://semver.org/}{\eweb} \\
\bottomrule
\end{tabular}
\end{table}

==> tables/data-auditing-1.tex <==
\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ \midrule

\multicolumn{4}{c}{\textsc{\emph{Data Auditing Tools}}} \\\midrule
\TextCircle\VisionCircle\EmptyCircle & \textbf{HaveIBeenTrained} & A combination search tool / opt out tool for LAION & \emojiblank\emojiblank\emojiblank\href{https://haveibeentrained.com/}{\eweb} \\

\midrule\multicolumn{4}{c}{\textsc{\emph{Data Auditing Case Studies}}} \\\midrule

\TextCircle\EmptyCircle\EmptyCircle & \textbf{A Datasheet for BookCorpus} & A third party datasheet for BookCorpus \citep{bandy2021addressing}. & \href{https://arxiv.org/abs/2105.05241}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Data Provenance Initiative} & A large scale audit of 2000+ popular datasets in AI \citep{longpre2023data}. & \href{https://arxiv.org/abs/2310.16787}{\earxiv}\href{https://huggingface.co/DataProvenanceInitiative}{\ehf}\href{https://github.com/Data-Provenance-Initiative/Data-Provenance-Collection}{\egithub}\href{https://www.dataprovenance.org/}{\eweb} \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Datasheet for the Pile} & A datasheet for the Pile \citep{biderman2022datasheet}. & \href{https://arxiv.org/abs/2201.07311}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\EmptyCircle & \textbf{Into the LAIONs Den} & Auditing hateful content in text-to-vision datasets \citep{birhane2023into}. & \href{https://arxiv.org/abs/2311.03449}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\EmptyCircle & \textbf{Multimodal dataset audit} & Auditing vision datasets for highly sensitive content, including misogyny, pornography and malignant stereotypes \citep{birhane2021multimodal}. & \href{https://arxiv.org/abs/2110.01963}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\EmptyCircle & \textbf{On Hate Scaling Laws} & Auditing text and vision datasets for systemic biases and hate \citep{birhane2023hate}. & \href{https://arxiv.org/abs/2306.13141}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Quality at a Glance} & An audit of allegedly multilingual parallel text corpora \citep{kreutzer2022quality}. & \href{https://arxiv.org/abs/2103.12028}{\earxiv}\emojiblank\emojiblank\emojiblank \\
%\TextCircle\VisionCircle\SpeechCircle & \textbf{Training Data Transparency Blog} & A blog on transparency for training data in AI. & \emojiblank\emojiblank\emojiblank\href{https://huggingface.co/blog/yjernite/data-transparency}{\eweb} \\


\bottomrule
\end{tabular}
\end{table}

==> tables/data-cleaning-1.tex <==
\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 
\midrule

    \multicolumn{4}{c}{\textsc{\emph{Dataset Cleaning \& Filtering}}} \\
    \midrule

\TextCircle\EmptyCircle\EmptyCircle & \textbf{Dolma's Toolkit} & A Python framework for defining Taggers that identify non-language text, language ID, PII, toxic text, and "quality" text. Includes reimplementation of heuristics used by Gopher and C4 for non-natural language \citep{dolma}. & \emojiblank\emojiblank\href{https://github.com/allenai/dolma}{\egithub}\emojiblank \\
\TextCircle\VisionCircle\EmptyCircle & \textbf{DataComp pre-filtering} & NSFW detection, dedup with eval datasets \citep{gadre2023datacomp}. & \href{https://arxiv.org/abs/2304.14108}{\earxiv}\href{https://huggingface.co/datasets/mlfoundations/datacomp_1b}{\ehf}\href{https://github.com/mlfoundations/dataset2metadata}{\egithub}\href{https://www.datacomp.ai/}{\eweb} \\
% \TextCircle\VisionCircle\EmptyCircle & \textbf{DataComp filtering} & Various quality filters \citep{gadre2023datacomp}. & \href{https://arxiv.org/abs/2304.14108}{\earxiv}\href{https://huggingface.co/datasets/mlfoundations/datacomp_1b}{\ehf}\href{https://github.com/mlfoundations/datacomp/tree/main#baselines}{\egithub}\href{https://www.datacomp.ai/}{\eweb} \\
% \TextCircle\EmptyCircle\EmptyCircle & \textbf{Data Selection via Importance Resampling (DSIR)} & A tool for selecting data with a similar distribution to a target dataset \citep{xie2023data}. & \href{https://arxiv.org/abs/2302.03169}{\earxiv}\emojiblank\href{https://github.com/p-lambda/dsir}{\egithub}\href{https://pypi.org/project/data-selection/}{\eweb} \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Lilac} & A python package for better understanding your data. Includes keyword and semantic search, as well as detection for PII, duplicates, and language. & \emojiblank\emojiblank\href{https://github.com/lilacai/lilac}{\egithub}\href{https://www.lilacml.com/}{\eweb} \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Roots data cleaning pipeline} & A pipeline for processing and improving quality of crowdsourced datasets \citep{NEURIPS2022_ce9e92e3}. & \href{https://arxiv.org/abs/2303.03915}{\earxiv}\emojiblank\href{https://github.com/bigscience-workshop/data-preparation/tree/main/preprocessing/training/01a_catalogue_cleaning_and_filtering}{\egithub}\emojiblank \\
% \TextCircle\EmptyCircle\EmptyCircle & \textbf{The Pile processing scripts} & A series of scripts to replicate the Pile dataset. Includes filtering and cleaning for: language, profanity, deduplication, and test set decontamination \citep{gao2020pile}. & \href{https://arxiv.org/abs/2101.00027}{\earxiv}\emojiblank\href{https://github.com/EleutherAI/the-pile/tree/master/processing_scripts}{\egithub}\emojiblank \\


    \midrule
    \multicolumn{4}{c}{\textsc{\emph{Language Identification}}} \\
    \midrule

\TextCircle\EmptyCircle\EmptyCircle & \textbf{Langdetect} & A tool to predict the language of text, used to filter out/in data from the desired languages. & \emojiblank\emojiblank\href{https://github.com/Mimino666/langdetect}{\egithub}\href{https://pypi.org/project/langdetect/}{\eweb} \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{fastText language classifier} & A tool for classifying the language of text \citep{grave2018learning}. & \href{https://arxiv.org/abs/1802.06893}{\earxiv}\href{https://huggingface.co/facebook/fasttext-language-identification}{\ehf}\emojiblank\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{FUN-LangID} & Frequently Used N-grams Language ID model, a character 4-gram model trained to recognize up to 1633 languages. & \emojiblank\emojiblank\href{https://github.com/google-research/url-nlp/tree/main/fun-langid}{\egithub}\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{OpenLID} & A model (and data used to train the model) for identifying 200+ languages \citep{Burchell_2023}. & \href{https://arxiv.org/abs/2305.13820}{\earxiv}\emojiblank\href{https://github.com/laurieburchell/open-lid-dataset}{\egithub}\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{GlotLID} & A model for identifying languages, with support for more than 1600 languages \citep{kargaran2023glotlid}. & \href{https://arxiv.org/abs/2310.16248}{\earxiv}\emojiblank\href{https://github.com/cisnlp/GlotLID}{\egithub}\emojiblank \\
% \TextCircle\EmptyCircle\EmptyCircle & \textbf{Detoxify} & A python library designed to identify toxic language in comments. Functions in seven languages: English, Italian, French, Russian, Portuguese, Spanish, Turking \citep{Hanu_Detoxify_2020}. & \emojiblank\emojiblank\href{https://github.com/unitaryai/detoxify}{\egithub}\emojiblank \\
% \TextCircle\EmptyCircle\EmptyCircle & \textbf{Dolma's Toolkit} & A Python framework for defining Taggers that identify non-language text, language ID, PII, toxic text, and "quality" text. Includes reimplementation of heuristics used by Gopher and C4 for non-natural language \citep{dolma}. & \emojiblank\emojiblank\href{https://github.com/allenai/dolma}{\egithub}\emojiblank \\
\EmptyCircle\EmptyCircle\SpeechCircle & \textbf{SpeechBrain’s Spoken language ID model} & Pre-trained spoken language identification model trained on VoxLingua107, dataset of audio sourced from YouTube for 107 languages \citep{ravanelli2021speechbrain}. & \href{https://arxiv.org/abs/2106.04624}{\earxiv}\href{https://huggingface.co/speechbrain/lang-id-voxlingua107-ecapa}{\ehf}\emojiblank\emojiblank \\

%     \midrule
%     \multicolumn{4}{c}{\textsc{\emph{Data Mixing}}} \\
%     \midrule

% \TextCircle\EmptyCircle\EmptyCircle & \textbf{DoReMi} & A github repository for \textbf{Do}main \textbf{Re}weighting with \textbf{Mi}nimax Optimization,  \citep{xie2023doremi}. & \href{https://arxiv.org/abs/2305.10429}{\earxiv}\emojiblank\href{https://github.com/sangmichaelxie/doremi}{\egithub}\emojiblank \\
% \TextCircle\EmptyCircle\EmptyCircle & \textbf{Online Data Mixing (ODM)} & A github repository for efficient online data mixing. \citep{albalak2023efficient}. & \href{https://arxiv.org/abs/2312.02406}{\earxiv}\emojiblank\href{https://github.com/alon-albalak/online-data-mixing}{\egithub}\emojiblank \\

\bottomrule
\end{tabular}
\end{table}

==> tables/data-decontamination-1.tex <==


\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 
\midrule

    \multicolumn{4}{c}{\textsc{\emph{Dataset Decontamination}}} \\
    \midrule

\TextCircle\EmptyCircle\EmptyCircle & \textbf{BigBench Canaries} & BigBench's "Training on the Test Set" Task provies guidance on using canaries to check if an evaluation set was trained on. & \emojiblank\emojiblank\href{https://github.com/google/BIG-bench/blob/main/bigbench/benchmark_tasks/training_on_test_set/README.md#training-on-the-test-set}{\egithub}\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Carper AI Decontamination Tool} & A repository, heavily based by the BigCode repository, to decontaminate evaluation sets from a text training set. & \emojiblank\emojiblank\href{https://github.com/CarperAI/decontamination/tree/main}{\egithub}\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Data Portraits} & A tool to test if a model has seen certain data, e.g. in the The Pile or The Stack \citep{marone2023data}. & \href{https://arxiv.org/abs/2303.03919}{\earxiv}\emojiblank\emojiblank\href{https://dataportraits.org/}{\eweb} \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Detect Data (Min-K Prob)} & A codebase that implements "Min-K\% Prob", a method to detect if a language model was pretrained on some text \citep{shi2023detecting}. & \href{https://arxiv.org/abs/2310.16789}{\earxiv}\emojiblank\href{https://github.com/swj0419/detect-pretrain-code}{\egithub}\href{https://swj0419.github.io/detect-pretrain.github.io/}{\eweb} \\
% \TextCircle\EmptyCircle\EmptyCircle & \textbf{Interpreting Canary Exposure} & An explanation on how to interpret canary exposure, including by relating it to membership inference attacks, and differential privacy \citep{jagielski2023note}. & \href{https://arxiv.org/abs/2306.00133}{\earxiv}\emojiblank\emojiblank\emojiblank \\
% \TextCircle\EmptyCircle\EmptyCircle & \textbf{Proving Test Set Contamination in Black Box Language Models} & A paper that provides methods for provable guarantees of test set contamination in language models without access to pretraining data or model weights \citep{oren2023proving}. & \href{https://arxiv.org/abs/2310.17623}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\bottomrule
\end{tabular}
\end{table}

==> tables/data-deduplication-1.tex <==
\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 
\midrule

    \multicolumn{4}{c}{\textsc{\emph{Dataset Deduplication}}} \\
    \midrule
\TextCircle\VisionCircle\SpeechCircle & \textbf{Apricot} & Apricot implements submodular optimization for summarizing massive datasets into minimally redundant subsets, useful for visualizing or deduplicating datasets \citep{JMLR:v21:19-467}. & \href{https://dl.acm.org/doi/abs/10.5555/3455716.3455877}{\earxiv}\emojiblank\href{https://github.com/jmschrei/apricot}{\egithub}\emojiblank \\
\EmptyCircle\VisionCircle\EmptyCircle & \textbf{DataComp} & Data to deduplicate vision datasets for the DataComp challenge \citep{gadre2023datacomp}. & \emojiblank\emojiblank\href{https://github.com/mlfoundations/dataset2metadata}{\egithub}\href{https://www.datacomp.ai/}{\eweb} \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Dolma's Toolkit} & Dolma uses a Bloom Filter implemented in Rust \citep{dolma}. & \emojiblank\emojiblank\href{https://github.com/allenai/dolma}{\egithub}\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Google Text Deduplication} & A repository to deduplicate language datasets \citep{lee-etal-2022-deduplicating}. & \href{https://arxiv.org/abs/2107.06499}{\earxiv}\emojiblank\href{https://github.com/google-research/deduplicate-text-datasets}{\egithub}\emojiblank \\
% \TextCircle\EmptyCircle\EmptyCircle & \textbf{RedPajama-Data} & Tools for: exact deduplication with bloom filter, fuzzy deduplication with LSH, calculating quality scores \citep{together_ai_2023_redpajama}. & \emojiblank\emojiblank\href{https://github.com/togethercomputer/RedPajama-Data}{\egithub}\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Pile Deduplication} & A set of tools for MinHashLSH deduplication \citep{gao2020pile}. & \href{https://arxiv.org/abs/2101.00027}{\earxiv}\emojiblank\href{https://github.com/EleutherAI/pile_dedupe}{\egithub}\emojiblank \\

\bottomrule
\end{tabular}
\end{table}




==> tables/data-documentation-1.tex <==
\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 
\midrule

    \multicolumn{4}{c}{\textsc{\emph{Data Documentation}}} \\
    \midrule

\TextCircle\VisionCircle\SpeechCircle & \textbf{Data Cards Playbook} & A tool to create a Data Card that thoroughly documents a new dataset \citep{pushkarna2022data}. & \href{https://dl.acm.org/doi/fullHtml/10.1145/3531146.3533231}{\earxiv}\emojiblank\emojiblank\href{https://sites.research.google/datacardsplaybook/}{\eweb} \\
% \TextCircle\VisionCircle\SpeechCircle & \textbf{Data Nutrition Labels} & A generic but thorough form of dataset documentation \citep{holland2020dataset}. & \href{https://arxiv.org/abs/1805.03677}{\earxiv}\emojiblank\emojiblank\href{https://datanutrition.org/}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Data Provenance Attribution Card} & A repository to select datasets and generate a summary. It can also generate a bibtex to attribute all developers of the datasets \citep{longpre2023data}. & \href{https://arxiv.org/abs/2310.16787}{\earxiv}\emojiblank\href{https://github.com/Data-Provenance-Initiative/Data-Provenance-Collection}{\egithub}\href{https://www.dataprovenance.org/}{\eweb} \\
% \TextCircle\VisionCircle\SpeechCircle & \textbf{Data Statements} & A data statement to thoroughly document a new dataset \citep{bender-friedman-2018-data}. & \href{https://aclanthology.org/Q18-1041/}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Datasheets for Datasets} & A datasheet to thoroughly document a new dataset \citep{gebru2021datasheets}. & \href{https://arxiv.org/abs/1803.09010}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Datasheets for Digital Cultural Heritage Datasets} & A datasheet specifically designed for digital cultural heritage datasets and their considerations \citep{alkemade2023datasheets}. & \href{https://cris.unibo.it/handle/11585/947893}{\earxiv}\emojiblank\emojiblank\emojiblank \\

\bottomrule
\end{tabular}
\end{table}

==> tables/data-governance-1.tex <==
\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 
\midrule\multicolumn{4}{c}{\textsc{\emph{Data Governance}}} \\\midrule
\TextCircle\VisionCircle\SpeechCircle & \textbf{Data Governance for BLOOM} & A paper detailing the data governance decisions undertaken during BigScience's BLOOM project. \cite{jernite2022data}.  & \href{https://dl.acm.org/doi/abs/10.1145/3531146.3534637}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Data Trusts for Training Data} & A paper that argues for the creation of a public data trust for collective input into the creation of AI systems and analyzes the feasibility of such a data trust. \cite{chan2023reclaiming}. & \href{https://arxiv.org/abs/2303.09001}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\EmptyCircle & \textbf{HaveIBeenTrained} & A combination search tool / opt out tool for LAION. & \emojiblank\emojiblank\emojiblank\href{https://haveibeentrained.com/}{\eweb} \\

\bottomrule
\end{tabular}
\end{table}

==> tables/data-search-1.tex <==


\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 
\midrule


    \multicolumn{4}{c}{\textsc{\emph{Pretraining Data Search \& Analysis}}} \\
    \midrule
\TextCircle\EmptyCircle\EmptyCircle & \textbf{AI2 C4 Search Tool} & A search tool that lets users to execute full-text queries to search Google's C4 Dataset. & \emojiblank\emojiblank\emojiblank\href{https://c4-search.apps.allenai.org/}{\eweb} \\
% \TextCircle\EmptyCircle\EmptyCircle & \textbf{GAIA Search Tool} & A search tool over C4, the Pile, ROOTS, and the text captions of LAION, developed with \href{https://github.com/castorini/pyserini}{Pyserini} \citep{piktus2023gaia} & \href{https://arxiv.org/abs/2306.01481}{\earxiv}\href{https://huggingface.co/spaces/spacerini/gaia}{\ehf}\emojiblank\emojiblank \\
\TextCircle\VisionCircle\EmptyCircle & \textbf{LAION search} & Nearest neighbor search based on CLIP embeddings. & \emojiblank\emojiblank\href{https://github.com/rom1504/clip-retrieval}{\egithub}\href{https://rom1504.github.io/clip-retrieval/}{\eweb} \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{ROOTS Search Tool} & A tool, based on a BM25 index, to search over text for each language or group of languages included in the ROOTS pretraining dataset \citep{piktus2023roots}. & \emojiblank\href{https://huggingface.co/spaces/bigscience-data/roots-search}{\ehf}\emojiblank\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{WIMBD} & A dataset analysis tool to count, search, and compare attributes across several massive pretraining corpora at scale, including C4, The Pile, and RedPajama \cite{elazar2023s}. & \href{https://arxiv.org/abs/2310.20707}{\earxiv}\emojiblank\href{https://github.com/allenai/wimbd}{\egithub}\href{https://wimbd.apps.allenai.org/}{\eweb} \\

    \midrule
    \multicolumn{4}{c}{\textsc{\emph{Finetuning Data Search \& Analysis}}} \\
    \midrule
% \TextCircle\EmptyCircle\EmptyCircle & \textbf{Data Finder} & A tool to help build search over academic datasets given a natural language description of the idea \citep{viswanathan2023datafinder}. & \href{https://arxiv.org/abs/2305.16636}{\earxiv}\emojiblank\href{https://github.com/viswavi/datafinder}{\egithub}\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Data Provenance Explorer} & An explorer tool for selecting, filtering, and visualizing popular finetuning, instruction, and alignment training datasets from Hugging Face, based on their metadata such as source, license, languages, tasks, topics, among other properties \cite{longpre2023data}. & \href{https://arxiv.org/abs/2310.16787}{\earxiv}\href{https://huggingface.co/DataProvenanceInitiative}{\ehf}\href{https://github.com/Data-Provenance-Initiative/Data-Provenance-Collection}{\egithub}\href{https://www.dataprovenance.org/}{\eweb} \\
% \TextCircle\EmptyCircle\EmptyCircle & \textbf{Hugging Face Data Measurements Tool} & A tool to analyze, measure, and compare properties of text finetuning data, including their distributional statistics, lengths, and vocabularies. & \emojiblank\href{https://huggingface.co/spaces/huggingface/data-measurements-tool}{\ehf}\emojiblank\emojiblank \\
\EmptyCircle\VisionCircle\EmptyCircle & \textbf{Know Your Data} & A tool for exploring over 70 vision datasets. & \emojiblank\emojiblank\href{https://github.com/PAIR-code/knowyourdata}{\egithub}\href{https://knowyourdata-tfds.withgoogle.com/}{\eweb} \\
\EmptyCircle\EmptyCircle\SpeechCircle & \textbf{NVIDIA Speech Data Explorer} & Tool for exploring speech data. & \emojiblank\emojiblank\emojiblank\href{https://docs.nvidia.com/deeplearning/nemo/user-guide/docs/en/stable/tools/speech_data_explorer.html}{\eweb} \\


\bottomrule
\end{tabular}
\end{table}

==> tables/environment-impact-1.tex <==
\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 
\midrule

    \multicolumn{4}{c}{\textsc{\emph{Estimating Environmental Impact}}} \\
    \midrule

\TextCircle\EmptyCircle\EmptyCircle & \textbf{Estimating the Carbon Footprint of BLOOM} & A comprehensive account of the broader environmental impact of the BLOOM language model \citep{luccioni2023estimating}. & \href{https://jmlr.org/papers/v24/23-0069.html}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Azure Emissions Impact Dashboard} & Monitoring the environmental impact of training machine learning models on Azure. & \emojiblank\emojiblank\emojiblank\href{https://www.microsoft.com/en-us/sustainability/emissions-impact-dashboard}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Carbontracker} & carbontracker is a tool for tracking and predicting the energy consumption and carbon footprint of training deep learning models \citep{anthony2020carbontracker}. & \href{https://arxiv.org/abs/2007.03051}{\earxiv}\emojiblank\href{https://github.com/lfwa/carbontracker}{\egithub}\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{CodeCarbon} & Estimate and track carbon emissions from your computer, quantify and analyze their impact \citep{schmidt2021codecarbon}. & \emojiblank\emojiblank\href{https://github.com/mlco2/codecarbon}{\egithub}\href{https://mlco2.github.io/codecarbon/}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Experiment Impact Tracker} & The experiment-impact-tracker is meant to be a drop-in method to track energy usage, carbon emissions, and compute utilization of your machine learning workload \cite{henderson2020towards}. & \href{https://arxiv.org/abs/2002.05651}{\earxiv}\emojiblank\href{https://github.com/Breakend/experiment-impact-tracker}{\egithub}\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Google Cloud Carbon Footprint Measurement} & Tracking the emissions of using Google's cloud compute resources. & \emojiblank\emojiblank\emojiblank\href{https://cloud.google.com/carbon-footprint?hl=en}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Making AI Less "Thirsty"} & Uncovering and Addressing the Secret Water Footprint of AI Models, and estimating water usage for training and deploying LLMs. & \href{https://arxiv.org/abs/2304.03271}{\earxiv}\emojiblank\href{https://github.com/Ren-Research/Making-AI-Less-Thirsty}{\egithub}\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{ML CO2 Impact} & A tool for estimating carbon impacts of ML training \citep{lacoste2019quantifying}. & \href{https://arxiv.org/abs/1910.09700}{\earxiv}\emojiblank\emojiblank\href{https://mlco2.github.io/impact/}{\eweb} \\

\bottomrule
\end{tabular}
\end{table}

==> tables/environment-impact-2.tex <==
\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 
\midrule

    \multicolumn{4}{c}{\textsc{\emph{Effective Use of Resources}}} \\
    \midrule

\TextCircle\EmptyCircle\EmptyCircle & \textbf{Scaling Laws for Neural Language Models} & Provide scaling laws to determine the optimal allocation of a fixed compute budget. & \href{https://arxiv.org/abs/2001.08361}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Training Compute-Optimal Large Language Models} & Provides details on the optimal model size and number of tokens for training a transformer-based language model in a given computational budget. & \href{https://arxiv.org/abs/2203.15556}{\earxiv}\emojiblank\emojiblank\emojiblank \\

\bottomrule
\end{tabular}
\end{table}

==> tables/finetuning-1.tex <==
\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 
\midrule


    \multicolumn{4}{c}{\textsc{\emph{Finetuning Data Catalogs}}} \\
    \midrule
\TextCircle\EmptyCircle\SpeechCircle & \textbf{Arabic NLP Data Catalogue} & A catalogue of hundreds of Arabic text and speech finetuning datasets, regularly updated. & \emojiblank\emojiblank\href{https://github.com/ARBML}{\egithub}\href{https://arbml.github.io/masader/}{\eweb} \\
% \TextCircle\EmptyCircle\EmptyCircle & \textbf{Aya Dataset Collection} & A permissively licensed multilingual instruction finetuning dataset curated by the Aya Annotation Platform from Cohere For AI. The dataset contains a total of 204k human-annotated prompt-completion pairs along with the demographics data of the annotators, spanning 65 languages \cite{singh2024aya}. & \href{https://arxiv.org/abs/2402.06619}{\earxiv}\href{https://huggingface.co/datasets/CohereForAI/aya_dataset}{\ehf}\emojiblank{\egithub}\href{https://cohere.com/research/aya}{\eweb} \\		
% \EmptyCircle\EmptyCircle\SpeechCircle & \textbf{CHiME-5} & Speaker Diarization dataset comprising over 50 hours of conversational speech recordings collected from twenty real dinner parties that have taken place in real homes & \emojiblank\emojiblank\emojiblank\href{https://licensing.sheffield.ac.uk/product/chime5}{\eweb} \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Data Provenance Collection} & An explorer tool for selecting popular finetuning, instruction, and alignment training datasets from Hugging Face, based on data provenance and characteristics criteria \cite{longpre2023data}. & \href{https://arxiv.org/abs/2310.16787}{\earxiv}\href{https://huggingface.co/DataProvenanceInitiative}{\ehf}\href{https://github.com/Data-Provenance-Initiative/Data-Provenance-Collection}{\egithub}\href{https://www.dataprovenance.org/}{\eweb} \\
\EmptyCircle\VisionCircle\EmptyCircle & \textbf{ImageNet} & An image classification dataset with 1.3M samples and 1000 classes \citep{russakovsky2015imagenet}. & \href{https://ieeexplore.ieee.org/abstract/document/5206848}{\earxiv}\emojiblank\emojiblank\href{https://www.image-net.org/}{\eweb} \\
% \TextCircle\EmptyCircle\SpeechCircle & \textbf{Indonesian NLP Data Catalogue} & A respository of hundreds of Indonesian language datasets. & \emojiblank\href{https://huggingface.co/NusaCrowd}{\ehf}\href{https://github.com/IndoNLP/nusa-crowd}{\egithub}\href{https://indonlp.github.io/nusa-catalogue/}{\eweb} \\
% \TextCircle\EmptyCircle\SpeechCircle & \textbf{Lanfrica} & An online catalogue that provides links to African language resources (papers and datasets) in both texts and speech & \emojiblank\emojiblank\emojiblank\href{https://lanfrica.com/}{\eweb} \\
\TextCircle\EmptyCircle\SpeechCircle & \textbf{Masakhane NLP} & A repository of African language text and speech resources, including datasets. & \emojiblank\href{https://huggingface.co/masakhane}{\ehf}\href{https://github.com/masakhane-io}{\egithub}\href{https://www.masakhane.io/}{\eweb} \\
\TextCircle\VisionCircle\EmptyCircle & \textbf{MS COCO} & Object detection, segemndation, captioning and retrieval dataset \citep{lin2014microsoft}. & \href{https://arxiv.org/abs/1405.0312}{\earxiv}\emojiblank\emojiblank\href{https://cocodataset.org/#home}{\eweb} \\
\EmptyCircle\EmptyCircle\SpeechCircle & \textbf{OpenSLR} & A collection of user-contributed datasets for various speech processing tasks. & \emojiblank\emojiblank\emojiblank\href{https://www.openslr.org/resources.php}{\eweb} \\
\TextCircle\EmptyCircle\SpeechCircle & \textbf{SEACrowd} & A repository of hundreds of South East Asian language datasets. & \emojiblank\emojiblank\href{https://github.com/SEACrowd}{\egithub}\href{https://seacrowd.github.io/seacrowd-catalogue/}{\eweb} \\
% \EmptyCircle\EmptyCircle\SpeechCircle & \textbf{VoxCeleb} & Speaker Identification dataset comprising of YouTube interviews from thousands of celebrities \citep{nagrani2017voxceleb}. & \href{https://arxiv.org/abs/1706.08612}{\earxiv}\emojiblank\emojiblank\href{https://www.robots.ox.ac.uk/~vgg/data/voxceleb/}{\eweb} \\
\EmptyCircle\EmptyCircle\SpeechCircle & \textbf{VoxLingua107} & Spoken language identification dataset created from YouTube videos, categroized by search phrases \citep{valk2021voxlingua107}. & \href{https://arxiv.org/abs/2011.12998}{\earxiv}\href{https://huggingface.co/speechbrain/lang-id-voxlingua107-ecapa}{\ehf}\emojiblank\href{https://bark.phon.ioc.ee/voxlingua107/}{\eweb} \\
\TextCircle\EmptyCircle\SpeechCircle & \textbf{Zenodo AfricaNLP Community} & An online catalogue that provides African language resources (data and models) in both texts and speech. & \emojiblank\emojiblank\emojiblank\href{https://zenodo.org/communities/africanlp}{\eweb} \\

\bottomrule
\end{tabular}
\end{table}

==> tables/general-capability-eval-1.tex <==
\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 
\midrule
\multicolumn{4}{c}{\textsc{\emph{Common Benchmarks for Text Capability Evaluation}}} \\
\midrule

\TextCircle\EmptyCircle\EmptyCircle & \textbf{BigBench} & A collaborative benchmark of 100s of tasks, probing LLMs on a wide array of unique capabilities \citep{srivastava2023beyond}. & \href{https://arxiv.org/abs/2206.04615}{\earxiv}\emojiblank\href{https://github.com/google/BIG-bench}{\egithub}\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{BigBench Hard} & A challenging subset of 23 BigBench tasks where 2022 models did not outperform annotator performance \citep{suzgun2022challenging}. & \href{https://arxiv.org/abs/2210.09261}{\earxiv}\emojiblank\href{https://github.com/suzgunmirac/BIG-Bench-Hard}{\egithub}\emojiblank \\

\TextCircle\EmptyCircle\EmptyCircle & \textbf{HELM classic} & A comprehensive suite of scenarios and metrics aimed at holistically evaluating models (including for capabilities) with comparisons to well known models \citep{liang2022holistic}. & \href{https://arxiv.org/abs/2211.09110}{\earxiv}\emojiblank\href{https://github.com/stanford-crfm/helm}{\egithub}\href{https://crfm.stanford.edu/helm/latest/}{\eweb} \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{HELM lite} & A lightweight subset of capability-centric benchmarks within HELM. Compares prominent open and closed models. & \href{https://crfm.stanford.edu/2023/12/19/helm-lite.html}{\earxiv}\emojiblank\href{https://github.com/stanford-crfm/helm}{\egithub}\href{https://crfm.stanford.edu/helm/lite/latest/#/}{\eweb} \\

\TextCircle\EmptyCircle\EmptyCircle & \textbf{LM Evaluation Harness} & Orchestration framework for standardizing LM prompted evaluation, supporting hundreds of subtasks. & \emojiblank\emojiblank\href{https://github.com/EleutherAI/lm-evaluation-harness}{\egithub}\href{https://github.com/EleutherAI/lm-evaluation-harness}{\eweb} \\

\TextCircle\EmptyCircle\EmptyCircle & \textbf{MMLU} & Evaluation of LM capabilities on multiple-choice college exam questions \citep{hendrycks2020measuring}. &\href{https://arxiv.org/pdf/2009.03300.pdf}{\earxiv}\href{https://huggingface.co/datasets/cais/mmlu}{\ehf}\href{https://github.com/hendrycks/test}{\egithub}\href{https://github.com/hendrycks/test#test-leaderboard}{\eweb} \\

\TextCircle\EmptyCircle\EmptyCircle & \textbf{MTEB} & The Massive Text Embedding Benchmark measures the quality of embeddings across 58 datasets and 112 languages for tasks related to retrieval, classification, clustering or semantic similarity. & \href{https://arxiv.org/abs/2210.07316}{\earxiv}\href{https://huggingface.co/spaces/mteb/leaderboard}{\ehf}\href{https://github.com/embeddings-benchmark/mteb}{\egithub}\emojiblank \\

\TextCircle\EmptyCircle\EmptyCircle & \textbf{SIB-200} & A large-scale open-sourced benchmark dataset for topic classification in 200 languages and dialects \citep{adelani2023sib}. & \href{https://arxiv.org/abs/2309.07445}{\earxiv}\href{https://huggingface.co/datasets/Davlan/sib200}{\ehf}\href{https://github.com/dadelani/sib-200	}{\egithub}\emojiblank \\	

\midrule
\multicolumn{4}{c}{\textsc{\emph{Common Benchmarks for Code Capability Evaluation}}} \\
\midrule

\TextCircle\EmptyCircle\EmptyCircle & \textbf{BigCode Evaluation Harness} & A framework for the evaluation of code generation models, compiling many evaluation sets. & \emojiblank\emojiblank\href{https://github.com/bigcode-project/bigcode-evaluation-harness/tree/main}{\egithub}\emojiblank \\

\TextCircle\EmptyCircle\EmptyCircle & \textbf{HumanEvalPack} & A code evaluation benchmark across 6 languages and 3 tasks, extending OpenAI's HumanEval \citep{muennighoff2023octopack}. & \href{https://arxiv.org/abs/2308.07124}{\earxiv}\href{https://huggingface.co/datasets/bigcode/humanevalpack}{\ehf}\href{https://github.com/bigcode-project/octopack}{\egithub}\emojiblank \\

\TextCircle\EmptyCircle\EmptyCircle & \textbf{SWE Bench} & SWE-bench is a benchmark for evaluating large language models on real world software issues collected from GitHub. Given a codebase and an issue, a language model is tasked with generating a patch that resolves the described problem \citep{jimenez2023swe}. & \href{https://arxiv.org/abs/2310.06770}{\earxiv}\emojiblank\href{https://github.com/princeton-nlp/SWE-bench}{\egithub}\href{https://www.swebench.com/}{\eweb} \\

\bottomrule
\end{tabular}
\end{table}

==> tables/general-capability-eval-2.tex <==
\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 
\midrule
\multicolumn{4}{c}{\textsc{\emph{Common Benchmarks for Multimodal Capability Evaluation}}} \\
\midrule

\TextCircle\VisionCircle\EmptyCircle & \textbf{CLIP benchmark} & Image classification, retrieval and captioning. & \emojiblank\emojiblank\href{https://github.com/LAION-AI/CLIP_benchmark}{\egithub}\emojiblank \\

\TextCircle\VisionCircle\EmptyCircle & \textbf{DataComp eval suite} & 38 image classification and retrieval downstream tasks \citep{gadre2023datacomp}. & \href{https://arxiv.org/abs/2304.14108}{\earxiv}\emojiblank\href{https://github.com/mlfoundations/datacomp#evaluation}{\egithub}\href{https://www.datacomp.ai/}{\eweb} \\

\TextCircle\VisionCircle\EmptyCircle & \textbf{HEIM} & A large suite of text-to-image evaluations. Useful for thorough capability analysis of these model types \citep{lee2023holistic}. & \href{https://arxiv.org/abs/2311.04287}{\earxiv}\emojiblank\emojiblank\href{https://crfm.stanford.edu/heim/v1.1.0/}{\eweb} \\

\EmptyCircle\EmptyCircle\SpeechCircle & \textbf{The Edinburgh International Accents of English Corpus} & Benchmark dataset of diverse English varieties for evaluating automatic speech recognition models (typically trained and tested only on US English) \citep{sanabria2023edinburgh}. & \href{https://arxiv.org/abs/2303.18110}{\earxiv}\emojiblank\emojiblank\href{https://groups.inf.ed.ac.uk/edacc/}{\eweb} \\

\TextCircle\VisionCircle\EmptyCircle & \textbf{MMBench} & A joint vision and text benchmark evaluating dozens of capabilities, using curated datasets and ChatGPT in the loop \citep{liu2023mmbench}. & \href{https://arxiv.org/abs/2307.06281}{\earxiv}\emojiblank\href{https://github.com/open-compass/MMBench}{\egithub}\href{https://opencompass.org.cn/mmbench}{\eweb} \\

\TextCircle\VisionCircle\EmptyCircle & \textbf{MME} & An evaluation benchmark for multimodal large language models with 14 manually curated subtasks, to avoid data leakage \citep{fu2023mme}. & \href{https://arxiv.org/abs/2306.13394}{\earxiv}\emojiblank\href{https://github.com/BradyFU/Awesome-Multimodal-Large-Language-Models/}{\egithub}\emojiblank \\

\TextCircle\VisionCircle\EmptyCircle & \textbf{MMMU} & A benchmark to evaluate joint text and vision models on 11k examples spanning 30 college-level subject domains \citep{yue2023mmmu}. & \href{https://arxiv.org/abs/2311.16502}{\earxiv}\href{https://huggingface.co/datasets/MMMU/MMMU}{\ehf}\href{https://github.com/MMMU-Benchmark/MMMU}{\egithub}\href{https://mmmu-benchmark.github.io/}{\eweb} \\

\TextCircle\VisionCircle\EmptyCircle & \textbf{OpenFlamingo eval suite} & VQA, captioning, classification evaluation suite \citep{awadalla2023openflamingo}. & \href{https://arxiv.org/abs/2308.01390}{\earxiv}\emojiblank\href{https://github.com/mlfoundations/open_flamingo/tree/main/open_flamingo/eval}{\egithub}\emojiblank \\

\midrule
\multicolumn{4}{c}{\textsc{\emph{Common Leaderboards for Capability Evaluation}}} \\
\midrule

\TextCircle\VisionCircle\SpeechCircle & \textbf{Hugging Face Leaderboards} & A set of popular model leaderboards on Hugging Face for ranking on generic metrics. & \emojiblank\href{https://huggingface.co/open-llm-leaderboard}{\ehf}\emojiblank\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{LMSys Chatbot Arena} & A leaderboard of models based on Elo ratings where humans or models select their preferred response between two anonymous models. Chatbot Arena, MT-Bench, and 5-shot MMLU are used as benchmarks. This resource provides a general purpose, and GPT-4 biased perspective into model capabilities \citep{zheng2023judging}. & \href{https://arxiv.org/abs/2306.05685}{\earxiv}\href{https://huggingface.co/spaces/lmsys/chatbot-arena-leaderboard}{\ehf}\href{https://github.com/lm-sys/FastChat/blob/main/docs/dataset_release.md}{\egithub}\emojiblank \\

\EmptyCircle\EmptyCircle\SpeechCircle & \textbf{OpenASR Leaderboard} & An automatic leaderboard ranking and evaluating speech recognition models on common benchmarks. & \emojiblank\href{https://huggingface.co/spaces/hf-audio/open_asr_leaderboard}{\ehf}\href{https://github.com/huggingface/open_asr_leaderboard}{\egithub}\emojiblank \\

\bottomrule
\end{tabular}
\end{table}

==> tables/harm-taxonomies-1.tex <==

\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\
\midrule
\multicolumn{4}{c}{\textsc{\emph{Harm Taxonomies}}} \\
\midrule



\TextCircle\VisionCircle\SpeechCircle & \textbf{Taxonomy of Harms} & Taxonomy of possible harms from generative AI systems to check your model against. & \emojiblank\emojiblank\emojiblank\href{https://arxiv.org/abs/2310.11986}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{A Holistic Approach to Undesired Content Detection in the Real World} & Description of five primary categories (Sexual, Hateful, Violent, Self-harm, Harassment) with sub-categories (e.g. Sexual / sexual content involving minors). Also describes a moderation filter (the OpenAI moderation endpoint), and releases a dataset labelled for the categories. & \href{https://arxiv.org/pdf/2208.03274.pdf}{\earxiv}\emojiblank\href{https://github.com/openai/moderation-api-release}{\egithub}\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{ActiveFence's LLM Safety Review: Benchmarks and Analysis} & Description of 4 risk categories, as part of a benchmark review of LLM safety: (1) Hate, (2) Misinformation, (3) Self-harm \& Suicide, (4) Child abuse \& exploitation. & \href{https://www.activefence.com/LLMSafety}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Red Teaming Language Models to Reduce Harms: Methods, Scaling Behaviors, and Lessons Learned} & Description of 20 risk areas, as part of red teaming Anthropics' models. Two of the tags are not interpretable ("Other" and "N/A - Invalid attempt"): Discrimination \& justice, Hate speech \& offensive language, Violence \& incitement, Non-violent unethical behaviour (e.g. lying, cheating), Bullying \& harassment, Other, Theft, N/A - Invalid attempt, Soliciting personally identifiable information, Conspiracy theories \& misinformation, Substance abuse \& banned substances, Fraud \& deception, Weapons, Adult content, Property crime \& vandalism, Animal abuse, Terrorism \& organized crime, Sexual exploitation \& human trafficking, Self-harm, Child abuse. & \href{https://arxiv.org/pdf/2209.07858.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{BEAVERTAILS: Towards Improved Safety Alignment of LLM via a Human-Preference Dataset} & Description of 14 risk areas, as part of a QA dataset for aligning models and evaluating their safety: Hate Speech, Offensive Language, Discrimination, Stereotype, Injustice, Violence, Aiding and Abetting, Incitement, Financial Crime, Property Crime, Theft, Privacy Violation, Drug Abuse, Weapons, Banned Substance, Non-Violent Unethical Behavior, Sexually Explicit, Adult Content, Controversial Topics, Politics, Misinformation Re. ethics, laws and safety, Terrorism, Organized Crime, Self-Harm, Animal Abuse, Child Abuse & \href{https://arxiv.org/pdf/2307.04657.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Safety Assessment of Chinese Large Language Models} & Description of 8 risk areas (called "safety scenarios)": Insult, Unfairness and Discrimination, Crimes and Illegal Activities, Sensitive Topics, Physical Harm, Mental health, Privacy and Property, Ethics and Morality. Six "instruction attacks" are also described: Goal hijacking, Prompt leaking, RolePlay Instruction, Unsafe Instruction Topic, Inquiry with Unsafe Opinion, Reverse Exposure. & \href{https://arxiv.org/pdf/2304.10436.pdf}{\earxiv}\emojiblank\href{https://github.com/thu-coai/Safety-Prompts}{\egithub}\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{DECODINGTRUST: A Comprehensive Assessment of Trustworthiness in GPT Models} & Description of 8 evaluation areas: toxicity, stereotypes bias, adversarial robustness, out-of-distribution robustness, robustness against adversarial demonstrations, privacy, machine ethics, fairness. & \href{https://arxiv.org/pdf/2306.11698.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{A Unified Typology of Harmful Content} & Taxonomy of harmful online content. There are 4 primary categories, which each have subcategories: (1) Hate and harassment (Doxxing, Identity attack, Identity misrepresentation, Insult, Sexual aggression, Threat of violence; (2) Self-inflicted harm (Eating disorder promotion, self-harm), (3) Ideological harm (Extremism Terrorism \& Organized crime, Misinformation), (4) Exploitation (Adult sexual services, Child sexual abuse material, Scams). & \href{https://aclanthology.org/2020.alw-1.16.pdf}{\earxiv}\emojiblank\emojiblank\href{https://docs.cohere.com/docs/content-moderation-with-classify}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Towards Safer Generative Language Models: A Survey on Safety Risks, Evaluations, and Improvements} & Description of 7 risk areas, as part of a survey on LLM risks: Toxicity and Abusive Content, Unfairness and Discrimination, Ethics and Morality Issues, Controversial Opinions, Misleading Information, Privacy and Data Leakage, Malicious Use and Unleashing AI Agents. & \href{https://arxiv.org/pdf/2302.09270.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Llama 2: Open Foundation and Fine-Tuned Chat Models} & Description of 3 risk areas, as part of the safety checks for releasing Llama2: (1) illicit and criminal activities (terrorism, theft, huam trafficking), (2) hateful and harmful activities (defamation, self-harm, eating disorders, discrimination), and (3) unqualified advice (medical, financial and legal advice). Other risk categories are described as part of red teaming and soliciting feedback. & \href{https://arxiv.org/pdf/2307.09288.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Ethical and social risks of harm from Language Models} & Two-tier taxonomy of risks, comprising both classification groups (of which there are 6) and associated harms (3 or 4 for each classification group). The classification groups are: (1) Discrimination, Exclusion and Toxicity, (2) Information Hazards, (3) Misinformation Harms, (4) Malicious Uses, (5) Human-Computer Interaction Harms, and (6) Automation, access, and environmental harms. & \href{https://arxiv.org/pdf/2112.04359.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Sociotechnical Safety Evaluation of Generative AI Systems} & Two-tier taxonomy of risks, comprising both classification groups (of which there are 6) and associated harms (3 or 4 for each classification group). The classification groups are: (1) Representation and Toxicity Harms, (2) Misinformation Harms, (3) Information \& Society Harms, (4) Malicious Use, (5) Human Autonomy \& Integrity Harms, and (6) Socioeconomic \& Environmental Harms. & \href{https://arxiv.org/pdf/2310.11986.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Trustworthy LLMs: a Survey and Guideline for Evaluating Large Language Models' Alignment} & Two-tier taxonomy of risks, with seven major categories of LLM trustworthiness, each of which has several associated sub-categories: (1) Reliability, (2) Safety, (3) Fairness, (4) Resistance to Misuse, (5) Explainability and Reasoning, (6) Social Norms, and (7) Robustness. & \href{https://arxiv.org/pdf/2308.05374.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Process for Adapting Language Models to Society (PALMS) with Values-Targeted Datasets} & Description of 8 risk areas, as part of describing methods for aligning models: (1) Abuse, Violence and Threat (inclusive of self-harm), (2) Health (phyiscal and mental), (3) Human characteristics and behaviour, (4) Injustice and inequality (incl, discrimination, harmful stereotypes), (5) Political opinion and destabilization, (6) Relationships (romantic, familial friendships), (7) Sexual activity (inclusive of pornography), (8) Terrorism (inclusive of white supremacy). & \href{https://arxiv.org/pdf/2106.10328.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Sociotechnical Harms of Algorithmic Systems: Scoping a Taxonomy for Harm Reduction} & Description of 5 categories of harm, with detailed subcategories: (1) Representational harms, (2) Allocative harms, (3) Quality of Service harms, (4) Interpersonal harms, and (5) Social system harms.  & \href{https://arxiv.org/pdf/2210.05791.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Deepfakes, Phrenology, Surveillance, and More! A Taxonomy of AI Privacy Risks} & Taxonomy of 12 privacy risks, based on reviewing 321 privacy-related incidents, filtered from the AI, Algorithmic and Automation Incident and Controversy Repository (AIAAIC) Database. Risks are split into those that are created by AI (Identification, Distortion, Exposure, Aggregation, Phrenology/Physiognomy) and those that are exacerbated by AI (Intrusion, Surveillance, Exclusion, Secondary Use, Insecurity, Increased Accessibility). & \href{https://arxiv.org/pdf/2310.07879.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\EmptyCircle\EmptyCircle\SpeechCircle & \textbf{The Ethical Implications of Generative Audio Models: A Systematic Literature Review} & Taxonomy of 12 "negative broader impacts" from generative models involving speech and music. & \href{https://arxiv.org/pdf/2307.05527.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{An Overview of Catastrophic AI Risks} & Taxonomy of 4 catastrophic AI risks, with subcategories: (1) Malicious use (Bioterrrorism, Uncontrolled AI agents, AI capabilities for propaganda, Censorship and surveillance), (2) AI race (Autonomous weapons,  Cyberwarfare, Automated human labour [mass unemployment and dependence on AI systems], (3) Organizational risks (AI accidentally leaked/stolen), (4) Rogue AIs (Proxy gaming, Goal drift, Power-seeking, Deception). & \href{https://arxiv.org/pdf/2306.12001.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{The Malicious Use of Artificial Intelligence: Forecasting, Prevention, and Mitigation} & Taxonomy of 3 AI security risks, with subcategories: (1) Digital Security, Physical Security, Political Security. & \href{https://img1.wsimg.com/blobby/go/3d82daa4-97fe-4096-9c6b-376b92c619de/downloads/MaliciousUseofAI.pdf?ver=1553030594217}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Open-sourcing highly capable foundation models} & Description of risks from malicious use of AI: Influence operations, Surveillance and population control, Scamming and spear phishing, Cyber attacks, Biological and chemical weapons development. Some "extreme risks" are also described in the paper (e.g. disruption to key societal functions). & \href{https://cdn.governance.ai/Open-Sourcing_Highly_Capable_Foundation_Models_2023_GovAI.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{How Does Access Impact Risk? Assessing AI Foundation Model Risk Along a Gradient of Access } & Description of risks from open-sourcing models, including five instances of malicious use: (1) Fraud and other crime schemes, (2) Undermining of social cohesion and democratic processes, (3) Human rights abuses, (4) Disruption of critical infrastructure, and (5) State conflict.  & \href{https://securityandtechnology.org/wp-content/uploads/2023/12/How-Does-Access-Impact-Risk-Assessing-AI-Foundation-Model-Risk-Along-A-Gradient-of-Access-Dec-2023.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{OpenAI Preparedness Framework (Beta)} & Description of 4 catastrophic AI risks: (1) Cybersecurity, (2) Chemical, Biological, Nuclear and Radiological (CBRN) threats, (3) Persuasion, and (4) Model autonomy. The paper also highlights the risk of "unknown unknowns". & \href{https://cdn.openai.com/openai-preparedness-framework-beta.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Anthropic's Responsible Scaling Policy} & Framework with four tiers of model capability, ffrom ASL-1 (smaller models) to ASL-4 (speculative), with increasing risk as models' capability increases. It also describes 4 catastrophic AI risks: (1) Misuse risks, (2) CBRN risks, (3) Cyber risks, and (4) Autonomy and replication risks. & \href{https://www-files.anthropic.com/production/files/responsible-scaling-policy-1.0.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Model evaluation for extreme risks} & Framework of 9 dangerous capabilities of AI models: (1) Cyber-offense, (2) Deception, (3) Persuasion \& manipulation, (4) Politial strategy, (5) Weapons acquisition, (6) Long-horizon planning, (7) AI development, (8) Situational awareness, (9) Self-proliferation. & \href{https://arxiv.org/pdf/2305.15324.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Frontier AI Regulation: Managing Emerging Risks to Public Safety} & Description of "sufficiently dangerous capabilities" of AI models to cause serious harm and disruption on a global scale, such as synthesing new biological or chemical weapons and evading human control through means of deception and obfuscation. & \href{https://arxiv.org/pdf/2307.03718.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{The Fallacy of AI Functionality} & Taxonomy of four AI failure points: (1) Impossible tasks (either Conceptually impossible or Practically impossible), (2) Engineering failures (Design failures, Implementation failures, Missing Safety Features), (3) Post-Deployment Failures (Robustness Issues, Failure under Adversarial Attacks, Unanticipated Intractions, (4) Communication Failures (Falsified or Overstated Capabilities, Misrepresented Capabilities). & \href{https://arxiv.org/pdf/2206.09511.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{TASRA: a Taxonomy and Analysis of Societal-Scale Risks from AI} & Framework of 3 potential harms from AI: (1) Harm to people (individual harm, Group/community harm, Societal harm), (2) Harm to an Organisation or Enterprise, (3) Harm to a system.  & \href{https://arxiv.org/pdf/2306.06924.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\

\bottomrule
\end{tabular}
\end{table}


==> tables/license-selection-1.tex <==

\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\
\midrule
\multicolumn{4}{c}{\textsc{\emph{General Guidance}}} \\
\midrule

\TextCircle\VisionCircle\SpeechCircle & \textbf{Behavioral Use Licensing for Responsible AI} & A paper that provides a theoretical framework for licenses intended for open models with use restrictions \citep{contractor2022behavioral}. & \href{https://dl.acm.org/doi/10.1145/3531146.3533143}{\earxiv}\emojiblank\emojiblank\emojiblank \\

\TextCircle\VisionCircle\SpeechCircle & \textbf{Legal Playbook For Natural Language Processing Researchers} & This playbook is a legal research resource for various activities related to data gathering, data governance, and disposition of an AI model available as a public resource. & \emojiblank\emojiblank\emojiblank\href{https://bigscience.huggingface.co/blog/legal-playbook-for-natural-language-processing-researchers}{\eweb} \\

\TextCircle\VisionCircle\SpeechCircle & \textbf{The Turning Way, Licensing} & A guide to reproducible research and licensing. & \emojiblank\emojiblank\emojiblank\href{https://the-turing-way.netlify.app/reproducible-research/licensing}{\eweb} \\


\bottomrule
\end{tabular}
\end{table}


\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\


\midrule
\multicolumn{4}{c}{\textsc{\emph{License Selection Guides}}} \\
\midrule

\TextCircle\VisionCircle\SpeechCircle & \textbf{Choose an open source license} & A guide for choosing among open source licenses that includes general selection criteria and explanations for software licenses. & \emojiblank\emojiblank\href{https://github.com/github/choosealicense.com/tree/gh-pages}{\egithub}\href{https://choosealicense.com/}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Creative Commons License Chooser} & A guide for choosing among Creative Commons licenses with an explanation of how they function. & \emojiblank\emojiblank\emojiblank\href{https://chooser-beta.creativecommons.org/}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Primer on AI2 ImpACT Licenses} & A post by AI2 describing when and why an organization should use a specific ImpACT license. & \emojiblank\emojiblank\emojiblank\href{https://allenai.org/impact-license}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Primer on RAIL Licenses} & A post by RAIL describing when and why an organization should use a specific RAIL license. & \emojiblank\emojiblank\emojiblank\href{https://oecd.ai/en/wonk/rails-licenses-trustworthy-ai}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{License Clause Comparison} & A comparison of behavioral use clauses included in foundation model licenses  \citep{mcduff2024standardization} & \href{https://arxiv.org/abs/2402.05979}{\earxiv}\emojiblank\emojiblank\emojiblank  \\

\midrule
\multicolumn{4}{c}{\textsc{\emph{Licenses}}} \\
\midrule

\TextCircle\VisionCircle\SpeechCircle & \textbf{Apache 2.0 License} & The most common open-source license for model weights. & \emojiblank\emojiblank\emojiblank\href{https://www.apache.org/licenses/LICENSE-2.0}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{AI2 ImpACT-LR License} & License for low risk AI artifacts (data and models) that allows for distribution of the artifact and its derivatives. Use restrictions include weapons development and military surveillance. & \emojiblank\emojiblank\emojiblank\href{https://allenai.org/licenses/impact-lr}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{AI2 ImpACT-MR License} & License for medium risk AI artifacts (data and models) that does not allows for distribution of the artifact but does allow for distribution of its derivatives. Use restrictions include weapons development and military surveillance. & \emojiblank\emojiblank\emojiblank\href{https://allenai.org/licenses/impact-mr}{\eweb} \\


\bottomrule
\end{tabular}
\end{table}



==> tables/model-documentation-1.tex <==

\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 
\midrule

    \multicolumn{4}{c}{\textsc{\emph{Model Documentation}}} \\
    \midrule

\TextCircle\VisionCircle\SpeechCircle & \textbf{Model Cards} & A standard for reporting and documenting machine learning models, for promoting and easing transparent and open model development or reporting \cite{mitchell2019model}. & \href{https://arxiv.org/abs/1810.03993}{\earxiv}\emojiblank\emojiblank\href{https://huggingface.co/spaces/huggingface/Model_Cards_Writing_Tool}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Model Card Resources} & A release of several resources surrounding model cards, including templates and tools for easy documentation creation, and how these are frequently used in practice. & \emojiblank\emojiblank\emojiblank\href{https://huggingface.co/blog/model-cards}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Ecosystem Cards} & Ecosystem Graphs centralize information about models and their impact in the broader ecosystem \cite{bommasani2023ecosystem}.  & \href{https://arxiv.org/abs/2303.15772}{\earxiv}\emojiblank\emojiblank\href{https://hai.stanford.edu/news/ecosystem-graphs-social-footprint-foundation-models}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Foundation Model Transparency Index} & An index to measure the transparency of a foundation model with respect to its inputs, development, and downstream uses or policies \cite{bommasani2023foundation}. & \href{https://arxiv.org/abs/2310.12941}{\earxiv}\emojiblank\href{https://github.com/stanford-crfm/fmti}{\egithub}\href{https://crfm.stanford.edu/fmti/}{\eweb} \\

\bottomrule
\end{tabular}
\end{table}





==> tables/model-training-1.tex <==
\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 
\midrule

    \multicolumn{4}{c}{\textsc{\emph{Pretraining Repositories}}} \\
    \midrule

\TextCircle\EmptyCircle\EmptyCircle & \textbf{GPT-NeoX} & A library for training large language models, built off Megatron-DeepSpeed and Megatron-LM with an easier user interface. Used at massive scale on a variety of clusters and hardware setups~\citep{gpt-neox-library}. & \emojiblank\emojiblank\href{https://github.com/EleutherAI/gpt-neox}{\egithub}\emojiblank \\

% \TextCircle\EmptyCircle\EmptyCircle & \textbf{Levanter} & A framework for training large language models (LLMs) and other foundation models that strives for legibility, scalability, and reproducibility. & \emojiblank\href{https://huggingface.co/stanford-crfm}{\ehf}\href{https://github.com/stanford-crfm/levanter}{\egithub}\href{https://crfm.stanford.edu/2023/06/16/levanter-1_0-release.html	}{\eweb} \\

% \TextCircle\EmptyCircle\EmptyCircle & \textbf{Megatron-LM} & One of the earliest open-source pretraining codebases for large language models. Still updated and has been used for a number of landmark distributed training and parallelism research papers by NVIDIA \citep{shoeybi2020megatronlm}. & \emojiblank\emojiblank\href{https://github.com/NVIDIA/Megatron-LM}{\egithub}\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Megatron-DeepSpeed} & A library for training large language models, built off of Megatron-LM but extended by Microsoft to support features of their DeepSpeed library \citep{smith2022using}. & \emojiblank\emojiblank\href{https://github.com/microsoft/Megatron-DeepSpeed}{\egithub}\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{OpenLM} & OpenLM is a minimal language modeling repository, aimed to facilitate research on medium sized LMs. They have verified the performance of OpenLM up to 7B parameters and 256 GPUs. They only depend only on PyTorch, XFormers, or Triton ~\citep{open_lm}. & \emojiblank\emojiblank\href{https://github.com/mlfoundations/open_lm}{\egithub}\emojiblank \\
\TextCircle\VisionCircle\EmptyCircle & \textbf{Kosmos-2} & For training multimodal models with CLIP backbones \citep{peng2023kosmos2}. & \href{https://arxiv.org/abs/2306.14824}{\earxiv}\href{https://huggingface.co/spaces/ydshieh/Kosmos-2}{\ehf}\href{https://github.com/microsoft/unilm/tree/master/kosmos-2}{\egithub}\emojiblank \\
\TextCircle\VisionCircle\EmptyCircle & \textbf{OpenCLIP} & Supports training and inference for over 100 CLIP models \citep{ilharco_gabriel_2021_5143773}. & \emojiblank\emojiblank\href{https://github.com/mlfoundations/open_clip}{\egithub}\emojiblank \\
\EmptyCircle\VisionCircle\EmptyCircle & \textbf{Pytorch Image Models (timm)} & Hub for models, scripts and pre-trained weights for image classification models. & \emojiblank\emojiblank\href{https://github.com/huggingface/pytorch-image-models}{\egithub}\emojiblank \\
\EmptyCircle\EmptyCircle\SpeechCircle & \textbf{Lhotse} & Python library for handling speech data in machine learning projects. & \emojiblank\emojiblank\emojiblank\href{https://github.com/lhotse-speech/lhotse}{\eweb} \\
\EmptyCircle\EmptyCircle\SpeechCircle & \textbf{Stable Audio Tools} & A codebase for distributed training of generative audio models. & \emojiblank\emojiblank\href{https://github.com/Stability-AI/stable-audio-tools}{\egithub}\emojiblank \\
\bottomrule
\end{tabular}
\end{table}

==> tables/model-training-2.tex <==
\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 
\midrule

    \multicolumn{4}{c}{\textsc{\emph{Finetuning Repositories}}} \\
    \midrule

\TextCircle\EmptyCircle\EmptyCircle & \textbf{Axolotl} & A repository for chat- or instruction-tuning language models, including through full fine-tuning, LoRA, QLoRA, and GPTQ. & \emojiblank\emojiblank\href{https://github.com/OpenAccess-AI-Collective/axolotl}{\egithub}\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Levanter} & A framework for training large language models (LLMs) and other foundation models that strives for legibility, scalability, and reproducibility. & \emojiblank\href{https://huggingface.co/stanford-crfm}{\ehf}\href{https://github.com/stanford-crfm/levanter}{\egithub}\href{https://crfm.stanford.edu/2023/06/16/levanter-1_0-release.html	}{\eweb} \\
\TextCircle\VisionCircle\EmptyCircle & \textbf{LLaMA-Adapter} & Fine-tuned LLMs on multimodal data using adapters \citep{gao2023llama}. & \href{https://arxiv.org/abs/2304.15010}{\earxiv}\emojiblank\href{https://github.com/OpenGVLab/LLaMA-Adapter}{\egithub}\emojiblank \\
% \TextCircle\VisionCircle\EmptyCircle & \textbf{BLIP-2} & Fine-tuned LLMs on multimodal data using a projection layer \citep{li2023blip2}. & \href{https://arxiv.org/abs/2301.12597}{\earxiv}\emojiblank\href{https://github.com/salesforce/LAVIS/tree/main/projects/blip2}{\egithub}\emojiblank \\
\TextCircle\VisionCircle\EmptyCircle & \textbf{LLaVA} & Fine-tuned LLMs on multimodal data using a projection layer \citep{liu2023improved}. & \href{https://arxiv.org/abs/2310.03744}{\earxiv}\href{https://huggingface.co/spaces/badayvedat/LLaVA}{\ehf}\href{https://github.com/haotian-liu/LLaVA}{\egithub}\href{https://llava-vl.github.io/}{\eweb} \\
% \TextCircle\VisionCircle\EmptyCircle & \textbf{MiniGPT4} & Fine-tuned LLMs on multimodal data using a projection layer \citep{zhu2023minigpt}. & \href{https://arxiv.org/abs/2304.10592}{\earxiv}\href{https://huggingface.co/spaces/Vision-CAIR/minigpt4}{\ehf}\href{https://github.com/Vision-CAIR/MiniGPT-4}{\egithub}\href{https://minigpt-4.github.io/}{\eweb} \\
% \TextCircle\VisionCircle\EmptyCircle & \textbf{OpenFlamingo} & Open source implementation of Flamingo \citep{awadalla2023openflamingo}. & \href{https://arxiv.org/abs/2308.01390}{\earxiv}\href{https://huggingface.co/openflamingo}{\ehf}\href{https://github.com/mlfoundations/open_flamingo}{\egithub}\href{https://laion.ai/blog/open-flamingo-v2/}{\eweb} \\
\TextCircle\VisionCircle\EmptyCircle & \textbf{Otter} & Multimodal models with Flamingo architecture \citep{li2023otterhd}. & \href{https://arxiv.org/abs/2311.04219}{\earxiv}\href{https://huggingface.co/spaces/Otter-AI/OtterHD-Demo}{\ehf}\href{https://github.com/Luodian/Otter}{\egithub}\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{peft} & A library for doing parameter efficient finetuning. & \emojiblank\emojiblank\href{https://github.com/huggingface/peft}{\egithub}\emojiblank \\
% \TextCircle\VisionCircle\SpeechCircle & \textbf{trl} & A library for doing RLHF. & \emojiblank\emojiblank\href{https://github.com/huggingface/trl}{\egithub}\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{trlX} & A library for doing RLHF at scale \citep{trlx-library}. & \href{https://aclanthology.org/2023.emnlp-main.530/}{\earxiv}\emojiblank\href{https://github.com/CarperAI/trlx}{\egithub}\href{https://trlx.readthedocs.io/en/latest/}{\eweb} \\


\bottomrule
\end{tabular}
\end{table}

==> tables/model-training-3.tex <==
\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 

\midrule\multicolumn{4}{c}{\textsc{\emph{Efficiency and Resource Allocation}}}\\\midrule

\TextCircle\VisionCircle\SpeechCircle & \textbf{Cerebras Model Lab} & A calculator to apply compute-optimal scaling laws for a given budget, including factoring expected total inference usage. & \emojiblank\emojiblank\emojiblank\href{https://www.cerebras.net/model-lab/}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{QLoRa} & An efficient finetuning approach that reduces memory usage while training \citep{dettmers2023qlora}. & \href{https://arxiv.org/abs/2305.14314}{\earxiv}\emojiblank\href{https://github.com/artidoro/qlora}{\egithub}\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Scaling Data-Constrained Language Models} & Demonstrates an optimal allocation of compute when dataset size is bounded \citep{muennighoff2023scaling}. & \href{https://arxiv.org/abs/2305.16264}{\earxiv}\href{https://huggingface.co/datablations}{\ehf}\href{https://github.com/huggingface/datablations}{\egithub}\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Training Compute-Optimal Language Models} & Proposes an optimal allocation of computational budget between model and dataset size, and shows experimental design for fitting scaling laws for compute allocation in a new setting \citep{hoffmann2022training}. & \href{https://arxiv.org/abs/2203.15556}{\earxiv}\emojiblank\emojiblank\emojiblank \\

\bottomrule
\end{tabular}
\end{table}

==> tables/model-training-4.tex <==
\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 
\midrule
\TextCircle\VisionCircle\SpeechCircle & \textbf{The EleutherAI Model Training Cookbook} & A set of resources on how to train large scale AI systems \citep{anthony2024cookbook}. & \emojiblank\emojiblank\href{https://github.com/EleutherAI/cookbook}{\egithub}\emojiblank \\
% \TextCircle\EmptyCircle\EmptyCircle & \textbf{Everything about Distributed Training and Efficient Finetuning} & A rundown and crash course in distributed training for deep learning, with an eye toward LLM finetuning and current useful tools and resources. Provides a good overview of the various (distributed) training strategies for efficient and scalable training. & \emojiblank\emojiblank\emojiblank\href{https://sumanthrh.com/post/distributed-and-efficient-finetuning/}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Machine Learning Engineering Online Book} & An "online textbook" and resource collection on ML engineering at scale, ranging from debugging distributed systems, parallelism strategies, effective use of large HPC clusters, and chronicles of past large-scale training runs with lessons learned. & \emojiblank\emojiblank\href{https://github.com/stas00/ml-engineering}{\egithub}\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{nanoGPT} & A minimal, stripped-down training codebase for teaching purposes and easily-hackable yet performant small-scale training. & \emojiblank\emojiblank\href{https://github.com/karpathy/nanoGPT}{\egithub}\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Transformer Inference Arithmetic} & A blog post on the inference costs of transformer-based LMs. Useful for providing more insight into deep learning accelerators and inference-relevant decisions to make when training a model. & \emojiblank\emojiblank\emojiblank\href{https://kipp.ly/transformer-inference-arithmetic/}{\eweb} \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Transformer Math 101} & An introductory blog post on training costs of LLMs, going over useful formulas and considerations from a high to low level. & \emojiblank\emojiblank\emojiblank\href{https://blog.eleuther.ai/transformer-math/}{\eweb} \\

    

\bottomrule
\end{tabular}
\end{table}

==> tables/old-model-training-1.tex <==
\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 
\midrule

    \multicolumn{4}{c}{\textsc{\emph{Model Training}}} \\
    \midrule

\TextCircle\EmptyCircle\EmptyCircle & \textbf{Training Compute-Optimal Language Models} & Proposes an optimal allocation of computational budget between model and dataset size, and shows experimental design for fitting scaling laws for compute allocation in a new setting. & \href{https://arxiv.org/abs/2203.15556}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Transformer Inference Arithmetic} & A blog post on the inference costs of transformer-based LMs. Useful for providing more insight into deep learning accelerators and inference-relevant decisions to make when training a model. & \emojiblank\emojiblank\emojiblank\href{https://kipp.ly/transformer-inference-arithmetic/}{\eweb} \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{nanoGPT} & A minimal, stripped-down training codebase for teaching purposes and easily-hackable yet performant small-scale training. & \emojiblank\emojiblank\href{https://github.com/karpathy/nanoGPT}{\egithub}\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Axolotl} & A repository for chat- or instruction-tuning language models, including through full fine-tuning, LoRA, QLoRA, and GPTQ. & \emojiblank\emojiblank\href{https://github.com/OpenAccess-AI-Collective/axolotl}{\egithub}\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Transformer Math 101} & An introductory blog post on training costs of LLMs, going over useful formulas and considerations from a high to low level & \emojiblank\emojiblank\emojiblank\href{https://blog.eleuther.ai/transformer-math/}{\eweb} \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Scaling Data-Constrained Language Models} & Demonstrates an optimal allocation of compute when dataset size is bounded & \href{https://arxiv.org/abs/2305.16264}{\earxiv}\href{https://huggingface.co/datablations}{\ehf}\href{https://github.com/huggingface/datablations}{\egithub}\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{GPT-NeoX} & A library for training large language models & \emojiblank\emojiblank\href{https://github.com/EleutherAI/gpt-neox}{\egithub}\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Megatron-DeepSpeed} & A library for training large language models & \emojiblank\emojiblank\href{https://github.com/microsoft/Megatron-DeepSpeed}{\egithub}\emojiblank \\
\TextCircle\VisionCircle\EmptyCircle & \textbf{OpenCLIP} & Supports training and inference for over 100 CLIP models & \emojiblank\emojiblank\href{https://github.com/mlfoundations/open_clip}{\egithub}\emojiblank \\
\TextCircle\VisionCircle\EmptyCircle & \textbf{BLIP-2} & Fine-tuned LLMs on multimodal data using a projection layer & \href{https://arxiv.org/abs/2301.12597}{\earxiv}\emojiblank\href{https://github.com/salesforce/LAVIS/tree/main/projects/blip2}{\egithub}\emojiblank \\
\TextCircle\VisionCircle\EmptyCircle & \textbf{OpenFlamingo} & Open source implementation of Flamingo & \href{https://arxiv.org/abs/2308.01390}{\earxiv}\href{https://huggingface.co/openflamingo}{\ehf}\href{https://github.com/mlfoundations/open_flamingo}{\egithub}\href{https://laion.ai/blog/open-flamingo-v2/}{\eweb} \\
\TextCircle\VisionCircle\EmptyCircle & \textbf{LLaMA-Adapter} & Fine-tuned LLMs on multimodal data using adapters & \href{https://arxiv.org/abs/2304.15010}{\earxiv}\emojiblank\href{https://github.com/OpenGVLab/LLaMA-Adapter}{\egithub}\emojiblank \\
\TextCircle\VisionCircle\EmptyCircle & \textbf{Otter} & Multimodal models with Flamingo architecture & \href{https://arxiv.org/abs/2311.04219}{\earxiv}\href{https://huggingface.co/spaces/Otter-AI/OtterHD-Demo}{\ehf}\href{https://github.com/Luodian/Otter}{\egithub}\emojiblank \\
\TextCircle\VisionCircle\EmptyCircle & \textbf{MiniGPT4} & Fine-tuned LLMs on multimodal data using a projection layer & \href{https://arxiv.org/abs/2304.10592}{\earxiv}\href{https://huggingface.co/spaces/Vision-CAIR/minigpt4}{\ehf}\href{https://github.com/Vision-CAIR/MiniGPT-4}{\egithub}\href{https://minigpt-4.github.io/}{\eweb} \\
\TextCircle\VisionCircle\EmptyCircle & \textbf{LLaVA} & Fine-tuned LLMs on multimodal data using a projection layer & \href{https://arxiv.org/abs/2310.03744}{\earxiv}\href{https://huggingface.co/spaces/badayvedat/LLaVA}{\ehf}\href{https://github.com/haotian-liu/LLaVA}{\egithub}\href{https://llava-vl.github.io/}{\eweb} \\
\TextCircle\VisionCircle\EmptyCircle & \textbf{Kosmos-2} & Multimodal models with CLIP backbones & \href{https://arxiv.org/abs/2306.14824}{\earxiv}\href{https://huggingface.co/spaces/ydshieh/Kosmos-2}{\ehf}\href{https://github.com/microsoft/unilm/tree/master/kosmos-2}{\egithub}\emojiblank \\
\EmptyCircle\VisionCircle\EmptyCircle & \textbf{Pytorch Image Models (timm)} & Hub for models, scripts and pre-trained weights for image classification & \emojiblank\emojiblank\href{https://github.com/huggingface/pytorch-image-models}{\egithub}\emojiblank \\
\EmptyCircle\EmptyCircle\SpeechCircle & \textbf{Lhotse} & Python library for handling speech data in machine learning projects & \emojiblank\emojiblank\emojiblank\href{https://github.com/lhotse-speech/lhotse}{\eweb} \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{QLoRa} & An efficient finetuning approach that reduces memory usage while training. & \href{https://arxiv.org/abs/2305.14314}{\earxiv}\emojiblank\href{https://github.com/artidoro/qlora}{\egithub}\emojiblank \\

\bottomrule
\end{tabular}
\end{table}



==> tables/pretraining-1.tex <==
\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 
\midrule
\multicolumn{4}{c}{\textsc{\emph{English Text}}} \\
    \midrule
    
    \TextCircle\EmptyCircle\EmptyCircle & \textbf{C4} & An English, cleaned version of \href{https://commoncrawl.org}{Common Crawl}'s web crawl corpus \citep{raffel2020exploring,dodge2021documenting}. & \href{https://arxiv.org/abs/1910.10683}{\earxiv}\href{https://huggingface.co/datasets/allenai/c4}{\ehf}\href{https://github.com/google-research/text-to-text-transfer-transformer#c4}{\egithub}\emojiblank \\
    
    \TextCircle\EmptyCircle\EmptyCircle & \textbf{Dolma} & An English-only pretraining corpus of 3 trillion tokens from a diverse mix of web content, academic publications, code, books, and encyclopedic materials \citep{soldaini2024dolma}. See the \href{https://github.com/allenai/dolma/blob/main/docs/assets/dolma-datasheet-v0.1.pdf}{datasheet}. & \href{https://arxiv.org/abs/2402.00159}{\earxiv}
    \href{https://huggingface.co/datasets/allenai/dolma}{\ehf}\href{https://github.com/allenai/dolma}{\egithub}\emojiblank \\

    \TextCircle\EmptyCircle\EmptyCircle & \textbf{The Pile} & An 825GB English pretraining corpus that mixes portions of common crawl with 22 smaller, high-quality datasets combined together \citep{gao2020pile,biderman2022datasheet}. & \href{https://arxiv.org/abs/2101.00027}{\earxiv}\href{https://huggingface.co/datasets/EleutherAI/pile}{\ehf}\emojiblank\href{https://pile.eleuther.ai/}{\eweb} \\

    % \TextCircle\EmptyCircle\EmptyCircle & \textbf{The RefinedWeb} & An English-only, web-only, deduplicated pretraining dataset of five trillion tokens \citep{penedo2023refinedweb}. & \href{https://arxiv.org/abs/2306.01116}{\earxiv}\href{https://huggingface.co/datasets/tiiuae/falcon-refinedweb}{\ehf}\emojiblank\emojiblank \\

    \midrule
    \multicolumn{4}{c}{\textsc{\emph{Multilingual Text}}} \\
    \midrule

    % \TextCircle\EmptyCircle\EmptyCircle & \textbf{mC4} & The multilingual cleaned version of \href{https://commoncrawl.org}{Common Crawl}'s web crawl corpus \citep{raffel2020exploring}. See this data analysis \cite{kreutzer2022quality}. & \href{https://arxiv.org/abs/1910.10683}{\earxiv}\href{https://huggingface.co/datasets/mc4}{\ehf}\emojiblank\emojiblank \\

    \TextCircle\EmptyCircle\EmptyCircle & \textbf{ROOTS} & A massive multilingual pretraining corpus from BigScience, comprised of 1.6TB of text spanning 59 languages \citep{laurenccon2022bigscience}. It is a mix of \href{https://oscar-project.org/}{OSCAR} \citep{laippala2022towards} and the datasets found in the BigScience Catalogue \citep{mcmillan2022documenting}. & \href{https://arxiv.org/abs/2303.03915}{\earxiv}\href{https://huggingface.co/bigscience-data}{\ehf}\href{https://github.com/bigscience-workshop/bigscience/tree/master/data}{\egithub}\href{https://bigscience.huggingface.co/}{\eweb} \\

    \TextCircle\EmptyCircle\EmptyCircle & \textbf{MADLAD-400} & An general domain 3T token monolingual dataset based on CommonCrawl, spanning 419 languages \citep{kudugunta2023madlad}. & \href{https://arxiv.org/abs/2309.04662}{\earxiv}\href{https://huggingface.co/datasets/allenai/MADLAD-400}{\ehf}\href{https://github.com/google-research/google-research/tree/master/madlad_400}{\egithub}\emojiblank \\
    
    \TextCircle\EmptyCircle\EmptyCircle & \textbf{RedPajama v2} & A pretraining dataset of 30 trillion deduplicated tokens from 84 CommonCrawl dumps and 5 languages \citep{together_ai_2023_redpajama}. & \emojiblank\href{https://huggingface.co/datasets/togethercomputer/RedPajama-Data-V2}{\ehf}\href{https://github.com/togethercomputer/RedPajama-Data}{\egithub}\href{https://www.together.ai/blog/redpajama-data-v2}{\eweb} \\
    
    \TextCircle\EmptyCircle\EmptyCircle & \textbf{CulturaX} & A pertaining dataset of 16T tokens, covering 167 languages, cleaned, deduplicated, and refined. Combines mC4 into 2020, with OSCAR project data up to 2023 \citep{nguyen2023culturax}. & \href{https://arxiv.org/abs/2309.09400}{\earxiv}\href{https://huggingface.co/datasets/uonlp/CulturaX}{\ehf}\emojiblank\emojiblank \\

    \TextCircle\EmptyCircle\EmptyCircle & \textbf{OSCAR} & The Open Super-large Crawled Aggregated coRpus provides web-based multilingual datasets across 166 languages \citep{suarez2019asynchronous,laippala2022towards}. & \href{https://aclanthology.org/2022.wnut-1.23/}{\earxiv}\emojiblank\emojiblank\href{https://oscar-project.org/}{\eweb} \\
    
    % \TextCircle\EmptyCircle\EmptyCircle & \textbf{OPUS} & The Open Parallel Corpus is a massive collection of translated text pairs from the web \citep{tiedemann2012parallel}. & \href{https://aclanthology.org/L12-1246/}{\earxiv}\emojiblank\emojiblank\href{https://opus.nlpl.eu/}{\eweb} \\

    \TextCircle\EmptyCircle\EmptyCircle & \textbf{WURA} & A manually audited multilingual pre-training corpus (document-level dataset) for 16 African languages and four  high-resource languages widely spoken in Africa (English, French, Arabic and Portuguese) \citep{oladipo-etal-2023-better}. & \href{https://aclanthology.org/2023.emnlp-main.11/}{\earxiv}\href{https://huggingface.co/datasets/castorini/wura}{\ehf}\emojiblank\emojiblank \\
    
\bottomrule
\end{tabular}
\end{table}

==> tables/pretraining-2.tex <==
\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 
\midrule
\multicolumn{4}{c}{\textsc{\emph{Specialized Text Pretraining Corpora}}} \\\midrule

    \TextCircle\EmptyCircle\EmptyCircle & \textbf{Open License Corpus} & The Open License Corpus is a 228B token corpus of permissively-licensed, English text data for pretraining \citep{min2023SILOLM}. & \href{https://arxiv.org/abs/2308.04430}{\earxiv}\href{https://huggingface.co/datasets/kernelmachine/open-license-corpus}{\ehf}\href{https://github.com/kernelmachine/silo-lm#download-data}{\egithub}\emojiblank \\
    
    \TextCircle\EmptyCircle\EmptyCircle & \textbf{Pile of Law} & An open-source, English dataset with 256GB of legal and administrative data, covering court opinions, contracts, administrative rules, and legislative records \citep{henderson2022pile}. & \href{https://arxiv.org/abs/2207.00220}{\earxiv}\href{https://huggingface.co/datasets/pile-of-law/pile-of-law}{\ehf}\emojiblank\emojiblank \\
    
    \TextCircle\EmptyCircle\EmptyCircle & \textbf{The Stack} & A 6TB permissively-licensed corpus from active GitHub repositories (358 programming languages) \citep{kocetkov2022stack}. & \href{https://arxiv.org/abs/2211.15533}{\earxiv}\href{https://huggingface.co/datasets/bigcode/the-stack}{\ehf}\href{https://github.com/bigcode-project/bigcode-dataset}{\egithub}\href{https://www.bigcode-project.org/docs/about/the-stack/#datasets-and-data-governance-tools-released-by-bigcode}{\eweb} \\
    
    \TextCircle\EmptyCircle\EmptyCircle & \textbf{The Proof Pile 2} & The Proof-Pile-2 is a 55 billion token dataset of mathematical and scientific documents \citep{azerbayev2023llemma}. & \href{https://arxiv.org/abs/2310.10631}{\earxiv}\href{https://huggingface.co/datasets/EleutherAI/proof-pile-2}{\ehf}\href{https://github.com/EleutherAI/math-lm}{\egithub}\href{https://blog.eleuther.ai/llemma/}{\eweb} \\
    
    % \TextCircle\EmptyCircle\EmptyCircle & \textbf{OpenWebMath} & A dataset containing the majority of the high-quality, mathematical text from the internet. It is filtered and extracted from over 200B HTML files on Common Crawl down to a set of 6.3 million documents containing a total of 14.7B tokens \citep{paster2023openwebmath}. & \href{https://arxiv.org/abs/2310.06786}{\earxiv}\href{https://huggingface.co/datasets/open-web-math/open-web-math}{\ehf}\href{https://github.com/keirp/OpenWebMath}{\egithub}\emojiblank \\
    
    \TextCircle\EmptyCircle\EmptyCircle & \textbf{peS2o} & A collection of ~40M creative open-access academic papers, cleaned, filtered, and formatted for pre-training of language models, originally derived from the Semantic Scholar Open Research Corpus (S2ORC) \citep{lo2020s2orc}. & \href{https://arxiv.org/abs/1911.02782}{\earxiv}\href{https://huggingface.co/datasets/allenai/peS2o}{\ehf}\emojiblank\emojiblank \\

\bottomrule
\end{tabular}
\end{table}

==> tables/pretraining-3.tex <==
\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 
\midrule


    \multicolumn{4}{c}{\textsc{\emph{Vision Pretraining Corpora}}} \\
    \midrule

    \TextCircle\VisionCircle\EmptyCircle & \textbf{LAION-5B} & A collection of over 5B image-text pairs collected from Common Crawl, optionally English-filtered \citep{schuhmann2022laion}. & \href{https://arxiv.org/abs/2210.08402}{\earxiv}\emojiblank\href{https://github.com/rom1504/img2dataset/blob/main/dataset_examples/laion5B.md}{\egithub}\href{https://laion.ai/blog/laion-5b/}{\eweb} \\
    \TextCircle\VisionCircle\EmptyCircle & \textbf{DataComp \& CommonPool} & A large pool of 13B image-text pairs from CommonCrawl and a curated 1B subset \citep{gadre2023datacomp}. & \href{https://arxiv.org/abs/2304.14108}{\earxiv}\href{https://huggingface.co/datasets/mlfoundations/datacomp_1b}{\ehf}\href{https://github.com/mlfoundations/datacomp}{\egithub}\href{https://www.datacomp.ai/}{\eweb} \\
    \TextCircle\VisionCircle\EmptyCircle & \textbf{MMC4} & Interleaved image-text data from Common Crawl (570M images, 43B tokens) \citep{zhu2023multimodal}. & \href{https://arxiv.org/abs/2304.06939}{\earxiv}\emojiblank\href{https://github.com/allenai/mmc4}{\egithub}\emojiblank \\
    \TextCircle\VisionCircle\EmptyCircle & \textbf{OBELICS} & Interleaved image-text data from Common Crawl (353 M images, 115B tokens) \citep{laurenccon2023obelisc}. & \href{https://arxiv.org/abs/2306.16527}{\earxiv}\href{https://huggingface.co/datasets/HuggingFaceM4/OBELICS}{\ehf}\href{https://github.com/huggingface/OBELICS}{\egithub}\href{https://huggingface.co/blog/idefics}{\eweb} \\

    \midrule
    \multicolumn{4}{c}{\textsc{\emph{Speech Pretraining Corpora}}} \\
    \midrule

\EmptyCircle\EmptyCircle\SpeechCircle & \textbf{Common Voice} & 28k hours of crowd-sourced read speech from 100+ languages. & \emojiblank\emojiblank\emojiblank\href{https://commonvoice.mozilla.org/en/datasets}{\eweb} \\
\EmptyCircle\EmptyCircle\SpeechCircle & \textbf{GigaSpeech} & 40k hours (10k transcribed) multi-domain English speech corpus \citep{chen2021gigaspeech}. & \href{https://arxiv.org/abs/2106.06909}{\earxiv}\emojiblank\href{https://github.com/SpeechColab/GigaSpeech}{\egithub}\emojiblank \\
\EmptyCircle\EmptyCircle\SpeechCircle & \textbf{Golos} & 1,240 hours of crowd-sourced Russian speech \citep{karpov2021golos}. & \href{https://arxiv.org/abs/2106.10161}{\earxiv}\emojiblank\href{https://github.com/sberdevices/golos}{\egithub}\href{https://www.openslr.org/114/}{\eweb} \\
\EmptyCircle\EmptyCircle\SpeechCircle & \textbf{IndicSUPERB} & 1,684 hour crowd-sourced corpus of 12 Indian languages \citep{javed2023indicsuperb}. & \href{https://arxiv.org/abs/2208.11761}{\earxiv}\emojiblank\emojiblank\href{https://ai4bharat.iitm.ac.in/indicsuperb/}{\eweb} \\
\EmptyCircle\EmptyCircle\SpeechCircle & \textbf{Libri-Light} & LibriVox English audiobooks (60k hours) \citep{kahn2020libri}. & \href{https://arxiv.org/abs/1912.07875}{\earxiv}\emojiblank\href{https://github.com/facebookresearch/libri-light}{\egithub}\emojiblank \\
% \EmptyCircle\EmptyCircle\SpeechCircle & \textbf{LibriSpeech} & 960 hour read English speech from LibriVox audiobooks \citep{panayotov2015librispeech}. & \href{http://www.danielpovey.com/files/2015_icassp_librispeech.pdf}{\earxiv}\emojiblank\emojiblank\href{https://www.openslr.org/12/}{\eweb} \\
\EmptyCircle\EmptyCircle\SpeechCircle & \textbf{The People’s Speech} & 30k hour conversational English dataset \citep{galvez2021people}. & \href{https://arxiv.org/abs/2111.09344}{\earxiv}\href{https://huggingface.co/datasets/MLCommons/peoples_speech}{\ehf}\emojiblank\emojiblank \\
% \EmptyCircle\EmptyCircle\SpeechCircle & \textbf{Samrómur} & 2,200 hour crowd-sourced corpus of Icelandic speech & \emojiblank\emojiblank\emojiblank\href{https://www.openslr.org/128/}{\eweb} \\
% \EmptyCircle\EmptyCircle\SpeechCircle & \textbf{Shrutilipi} & 6,400 hour corpus of TV/Radio broadcasts from 12 Indian languages & \href{https://arxiv.org/abs/2208.12666}{\earxiv}\emojiblank\emojiblank\href{https://ai4bharat.iitm.ac.in/shrutilipi/}{\eweb} \\
\EmptyCircle\EmptyCircle\SpeechCircle & \textbf{VoxPopuli} & 400k hours of unlabelled speech from 23 languages of the European parliament \citep{wang2021voxpopuli}. & \href{https://arxiv.org/abs/2101.00390}{\earxiv}\emojiblank\href{https://github.com/facebookresearch/voxpopuli}{\egithub}\emojiblank \\
\EmptyCircle\EmptyCircle\SpeechCircle & \textbf{WenetSpeech} & 22.4k hour multi-domain corpus of Mandarin \citep{zhang2022wenetspeech}. & \href{https://arxiv.org/abs/2110.03370}{\earxiv}\emojiblank\href{https://github.com/wenet-e2e/WenetSpeech}{\egithub}\href{https://www.openslr.org/121/}{\eweb} \\

\bottomrule
\end{tabular}
\end{table}

==> tables/review.tex <==
% \begin{table*}[t!]
% \centering
% \footnotesize
% % \renewcommand{\arraystretch}{1.5}
% \begin{adjustbox}{width=\textwidth}
% \begin{tabular}{p{3cm} p{13cm}}
% \toprule
% \textbf{Section} & \textbf{Review Summary}\\
% \midrule

% \multirow{4}{*}{Data Sources} & The community would benefit from more accurate and comprehensive licensing, provenance, and creator consent information for existing datasets. \\
% & \cellcolor[gray]{0.9}The community would benefit from more accurate and comprehensive information on sensitive content, such
% as CSAM and NCII. \\
% & Data \& modeling have focused predominantly on easy-to-scale data formats, neglecting other formats. \\
% & \cellcolor[gray]{0.9}There is a scarcity of realistic training tasks, and naturalistic observations. \\
% \midrule
% \multirow{6}{*}{Data Preparation} & Placeholder. \\
% & \cellcolor[gray]{0.9}Placeholder. \\
% & Placeholder. \\
% & \cellcolor[gray]{0.9}Placeholder. \\
% & Placeholder. \\
% & \cellcolor[gray]{0.9}Placeholder. \\
% \midrule
% \multirow{3}{*}{Data Documentation \& Release} & Placeholder. \\
% & \cellcolor[gray]{0.9}Placeholder. \\
% & Placeholder. \\
% \midrule
% \multirow{4}{*}{Model Training} & Placeholder. \\
% & \cellcolor[gray]{0.9}Placeholder. \\
% & Placeholder. \\
% & \cellcolor[gray]{0.9}Placeholder. \\
% \midrule
% \multirow{5}{*}{Environmental Impact} & Transparency from consumer-level API providers, into query-level energy and environmental usage measures. \\
% & \cellcolor[gray]{0.9}Transparency from hardware makers and data centers, into fine-grained energy and environmental usage measures. \\
% & ``Energy Star'' standards for non-technical users to fairly compare AI services. \\
% & \cellcolor[gray]{0.9}Scaling laws research currently lacks empirical evidence for the new wave of multi-modal models, and intuitive user interfaces for new developers. \\
% \midrule
% \multirow{1}{*}{Model Evaluation} & Placeholder \\
% \midrule
% \multirow{1}{*}{Model Release \& Monitoring} & Placeholder \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \caption{\textbf{A summary of the reviews \& take-aways from each phase of foundation model development ecosystem.}}
% \label{tab:review-summary}
% \end{table*}

\begin{table*}[t!]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.5} % Adjusting vertical space between rows
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{m{3cm} m{13cm}} % Changed from p to m for vertical centering
\toprule
\textbf{Section} & \textbf{Review Summary}\\
\midrule

\multirow{4}{*}{Data Sources} & The community would benefit from more accurate and comprehensive licensing, provenance, and creator consent information for existing datasets. \\
& \cellcolor[gray]{0.9}The community would benefit from more accurate and comprehensive information on sensitive content, such as CSAM and NCII. \\
& Data \& modeling have focused predominantly on easy-to-scale data formats, neglecting other formats. \\
& \cellcolor[gray]{0.9}There is a scarcity of realistic training tasks, and naturalistic observations. \\
\midrule
\multirow{5}{*}{Data Preparation} &The community stands to benefit greatly from increased efforts on open-source data exploration tools. \\
& \cellcolor[gray]{0.9} Open-source data exploration tools allow for retrospective analysis of datasets. \\
& Consolidating on a standardized format for data storage and processing will give developers more time to focus on developing infrastructure. \\
& \cellcolor[gray]{0.9} Developing data-centric benchmarks can catalyze progress. \\
& Data preparation tools should consider not only English-centric data, but non-English and low-resource languages. \\
\midrule
\multirow{3}{*}{Data Documentation} & Data documentation is essential for reproducibility, avoiding misuse, and helping downstream users build constructively on prior work. \\
% Data Documentation \& Release & Placeholder. \\
& \cellcolor[gray]{0.9} The documentation process should be started early, as data is collected and processed. \\
& For datasets with multiple stakeholders, or derived from community efforts, it is important to appropriately proactively organize its access, licenses, and stewardship. \\
\midrule
\multirow{4}{*}{Model Training} & More resources, especially non-English ones, for lowering the barrier to entry for less technical developers are needed. \\
& \cellcolor[gray]{0.9} More standardized and centralized resources, especially cross-modality, should be focused on in the future. \\
& Other options for massively collaborative model development should be pursued. \\
\midrule
\multirow{5}{*}{Environmental Impact} & Transparency from consumer-level API providers, into query-level energy and environmental usage measures. \\
& \cellcolor[gray]{0.9}Transparency from hardware makers and data centers, into fine-grained energy and environmental usage measures. \\
& ``Energy Star'' standards for non-technical users to fairly compare AI services. \\
& \cellcolor[gray]{0.9}Scaling laws research currently lacks empirical evidence for the new wave of multi-modal models, and intuitive user interfaces for new developers. \\
\midrule
\multirow{3}{*}{Model Evaluation} & Placeholder \\
& \cellcolor[gray]{0.9} Placeholder \\
& Placeholder \\
\midrule
\multirow{3}{*}{Model Release} & \cellcolor[gray]{0.9}Models should be released with accompanying documentation \emph{and} easy-to-run code for training, evaluation and inference. \\
& Developers should be thoughtful about the type of license to use for artifacts and whether to include behavioral use clauses. \\
&  \cellcolor[gray]{0.9} Frameworks for monitoring and shaping model usage have become more prevalent; however, more tooling and support is needed. \\

\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{A summary of the reviews \& take-aways from each phase of foundation model development ecosystem.}}
\label{tab:review-summary}
\end{table*}

% \citet{yang2023shadow} & Safety and security & Safety alignment can be subverted with minimal finetuning.
% \\ \rowcolor[gray]{0.9}
% \citet{choi2023tools} & Privacy and security & Assessing the ability to verify a model's training data.
% \\
% \citet{patil2023can} & Privacy and security & Methods to prevent sensitive information extraction attacks.
% \\ \rowcolor[gray]{0.9}
% \citet{zou2023universal} & Safety and alignment & Adversarial attacks that transfer from open models to black-box, closed models.
% \\ 

==> tables/risks-harms-1.tex <==
\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 
\midrule

    \multicolumn{4}{c}{\textsc{\emph{Risk Evaluation Overviews}}} \\
    \midrule

% \TextCircle\VisionCircle\SpeechCircle & \textbf{Taxonomy of Harms} & Taxonomy of possible harms from generative AI systems to check your model against. & \emojiblank\emojiblank\emojiblank\href{https://arxiv.org/abs/2310.11986}{\eweb} \\
\TextCircle & \textbf{SafetyPrompts website} & Open repository of datasets for LLM evaluation and mitigation. & \emojiblank\emojiblank\emojiblank\href{https://safetyprompts.com/}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Safety evaluation repository} & A repository of 200+ safety evaluations, across modalities and harms. Useful for delving deeper into the array of risks. & \emojiblank\emojiblank\emojiblank\href{https://dpmd.ai/46CPd58}{\eweb} \\

    \midrule
    \multicolumn{4}{c}{\textsc{\emph{Bias \& Toxicity Evaluations}}} \\
    \midrule
    
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Bias Benchmark for QA (BBQ)} & A dataset of question-sets constructed by the authors that highlight attested social biases against people belonging to protected classes along nine different social dimensions relevant for U.S. English-speaking contexts \citep{parrish2021bbq}. & \href{https://arxiv.org/abs/2110.08193}{\earxiv}\emojiblank\href{https://github.com/nyu-mll/BBQ}{\egithub}\emojiblank \\
\TextCircle\VisionCircle\EmptyCircle & \textbf{Crossmodal-3600} & Image captioning evaluation with geographically diverse images in 36 languages \citep{thapliyal2022crossmodal}. & \href{https://arxiv.org/abs/2205.12522}{\earxiv}\emojiblank\href{https://google.github.io/crossmodal-3600/}{\egithub}\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{HolisticBias} & A bias and toxicity benchmark using templated sentences, covering nearly 600 descriptor terms across 13 different demographic axes, for a total of 450k examples \citep{smith2022m}. & \href{https://arxiv.org/abs/2205.09209}{\earxiv}\emojiblank\href{https://github.com/facebookresearch/ResponsibleNLP/tree/main/holistic_bias}{\egithub}\href{https://ai.meta.com/research/publications/im-sorry-to-hear-that-finding-new-biases-in-language-models-with-a-holistic-descriptor-dataset/}{\eweb} \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{RealToxicityPrompts} & 100k web sentence snippets for researchers to assess the risk of neural toxic degeneration in models \citep{gehman2020realtoxicityprompts}. & \href{https://arxiv.org/abs/2009.11462}{\earxiv}\emojiblank\href{https://github.com/allenai/real-toxicity-prompts}{\egithub}\href{https://toxicdegeneration.allenai.org/}{\eweb} \\
\EmptyCircle\VisionCircle\EmptyCircle & \textbf{StableBias} & Bias testing benchmark for Image to Text models, based on gender-occupation associations \citep{luccioni2023stable}. & \href{https://arxiv.org/abs/2303.11408}{\earxiv}\href{https://huggingface.co/spaces/society-ethics/StableBias}{\ehf}\emojiblank\emojiblank \\


    \midrule
    \multicolumn{4}{c}{\textsc{\emph{Factuality Evaluations}}} \\
    \midrule

\TextCircle\EmptyCircle\EmptyCircle & \textbf{FactualityPrompt} & A benchmark to measure factuality in language models \citep{lee2022factuality}. & \href{https://arxiv.org/abs/2206.04624}{\earxiv}\emojiblank\href{https://github.com/nayeon7lee/FactualityPrompt}{\egithub}\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Hallucinations} & Public LLM leaderboard computed using Vectara's Hallucination Evaluation Model. It evaluates LLM hallucinations when summarizing a document \citep{Hughes-Vectara-Hallucination-Leaderboard-2023}.  & \emojiblank\href{https://huggingface.co/vectara/hallucination_evaluation_model}{\ehf}\emojiblank\href{https://github.com/vectara/hallucination-leaderboard}{\eweb} \\
% \TextCircle\EmptyCircle\EmptyCircle & \textbf{Head-to-Tail} & For knowledge testing: a benchmark that consists of 18K question-answer (QA) pairs regarding head, torso, and tail facts in terms of popularity \citep{sun2023head}.  & \href{https://arxiv.org/abs/2308.10168}{\earxiv}\emojiblank\emojiblank\href{https://paperswithcode.com/paper/head-to-tail-how-knowledgeable-are-large}{\eweb} \\

% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[H]
% % \begin{tabular}{@{}lllll@{}}
% \begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
% \toprule
% \textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\
    \midrule
    \multicolumn{4}{c}{\textsc{\emph{Information \& Safety Hazard Evaluations}}} \\
    \midrule

\TextCircle\EmptyCircle\EmptyCircle & \textbf{Purple Llama CyberSecEval} & A benchmark for coding assistants, measuring their propensity to generate insecure code and level of compliance when asked to assist in cyberattacks \citep{bhatt2023purple}. & \href{https://arxiv.org/abs/2312.04724}{\earxiv}\emojiblank\href{https://github.com/facebookresearch/PurpleLlama/tree/main/CybersecurityBenchmarks}{\egithub}\href{https://ai.meta.com/research/publications/purple-llama-cyberseceval-a-benchmark-for-evaluating-the-cybersecurity-risks-of-large-language-models/}{\eweb} \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{Purple Llama Guard} & A tool to identify and protect against malicious inputs to LLMs \citep{inan2023llama}. & \href{https://arxiv.org/abs/2312.06674}{\earxiv}\emojiblank\href{https://github.com/facebookresearch/PurpleLlama/tree/main/Llama-Guard}{\egithub}\href{https://ai.meta.com/research/publications/llama-guard-llm-based-input-output-safeguard-for-human-ai-conversations/}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{OpenAI content moderation filter} & A moderation filter and released dataset. The endpoint has 5 primary categories (Sexual, Hateful, Violent, Self-harm, Harassment) with sub-categories. & \href{https://arxiv.org/pdf/2208.03274.pdf}{\earxiv}\emojiblank\href{https://github.com/openai/moderation-api-release}{\egithub}\emojiblank \\
%\TextCircle\EmptyCircle\EmptyCircle & \textbf{Red Teaming LMs with LMs} & A method for using one language model to automatically find cases where a target LM behaves in a harmful way, by generating test cases \citep{perez2022red}. & \href{https://arxiv.org/abs/2202.03286}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\EmptyCircle\EmptyCircle & \textbf{SimpleSafetyTests} & Small probe set (100 English text prompts) covering severe harms: child abuse, suicide, self-harm and eating disorders, scams and fraud, illegal items, and physical harm \citep{vidgen2023simplesafetytests}. & \href{https://arxiv.org/abs/2311.08370}{\earxiv}\emojiblank\href{https://github.com/bertiev/SimpleSafetyTests}{\egithub}\emojiblank \\

\bottomrule
\end{tabular}
\end{table}

==> tables/risks-harms-taxonomies-1.tex <==
\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\ 
\midrule

    \multicolumn{4}{c}{\textsc{\emph{Taxonomies of Risk and Harm}}} \\
    \midrule




\TextCircle\VisionCircle\SpeechCircle & \textbf{Ethical and social risks of harm from language models} & A two-level taxonomy of LLM risks, comprising both classification groups and associated harms \citep{weidinger2021ethical}. The classification groups are: (1) Discrimination, Exclusion and Toxicity, (2) Information Hazards, (3) Misinformation Harms, (4) Malicious Uses, (5) Human-Computer Interaction Harms, and (6) Automation, access, and environmental harms. & \href{https://arxiv.org/pdf/2112.04359.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Taxonomy of Risks posed by Language Models} & A taxonomy of language model risks \citep{10.1145/3531146.3533088}. The classification groups are: (1) Discrimination, Hate speech and Exclusion, (2) Information Hazards, (3) Misinformation Harms, (4) Malicious Uses, (5) Human-Computer Interaction Harms, and (6) Environmental and Socioeconomic harms. For each risk area, the authors describe relevant evidence, causal mechanisms, and risk mitigation approaches. & \href{https://arxiv.org/pdf/2112.04359.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Sociotechnical Safety Evaluation of Generative AI Systems} & A two-level taxonomy of AI risks, comprising both classification groups and associated harms \citep{weidinger2023sociotechnical}. The classification groups are: (1) Representation and Toxicity Harms, (2) Misinformation Harms, (3) Information \& Society Harms, (4) Malicious Use, (5) Human Autonomy \& Integrity Harms, and (6) Socioeconomic \& Environmental Harms. & \href{https://arxiv.org/pdf/2310.11986.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Sociotechnical Harms of Algorithmic Systems} & A taxonomy of AI harms with detailed subcategories, focused on mitigating harm \citep{shelby2023sociotechnical}. The harm categories are: (1) Representational harms, (2) Allocative harms, (3) Quality of Service harms, (4) Interpersonal harms, and (5) Social system harms.  & \href{https://arxiv.org/pdf/2210.05791.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Assessing Language Model Deployment with Risk Cards} & A framework for structured assessment and documentation of risks associated with applications of language models \citep{derczynski2023assessing}. Each RiskCard makes clear the routes for the risk to manifest harm, their placement in harm taxonomies, and example prompt-output pairs. 70+ risks are identified, based on a literature survey.& \href{https://arxiv.org/pdf/2303.18190.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{An Overview of Catastrophic AI Risks} & A taxonomy of 4 catastrophic AI risks, with associated subcategories \citep{hendrycks2023overview}: (1) Malicious use,(2) AI race,(3) Organizational risks, (4) Rogue AIs (Proxy gaming, Goal drift, Power-seeking, Deception). & \href{https://arxiv.org/pdf/2306.12001.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{OpenAI Preparedness Framework} & Description of 4 catastrophic AI risks \citep{openai2023preparedness}: (1) Cybersecurity, (2) Chemical, Biological, Nuclear and Radiological (CBRN) threats, (3) Persuasion, and (4) Model autonomy. The paper also highlights the risk of "unknown unknowns". & \href{brundage2018malicious}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Model evaluation for extreme risks} & A framework of 9 dangerous capabilities of AI models  \citep{shevlane2023model}: (1) Cyber-offense, (2) Deception, (3) Persuasion \& manipulation, (4) Political strategy, (5) Weapons acquisition, (6) Long-horizon planning, (7) AI development, (8) Situational awareness, (9) Self-proliferation. & \href{https://arxiv.org/pdf/2305.15324.pdf}{\earxiv}\emojiblank\emojiblank\emojiblank \\
\bottomrule
\end{tabular}
\end{table}

==> tables/usage-monitoring-1.tex <==

\begin{table}[H]
% \begin{tabular}{@{}lllll@{}}
\begin{tabular}{@{}p{\colOneSize}p{\colTwoSize}p{\colThreeSize}p{\colFourSize}@{}}
\toprule
\textsc{Modality} & \textsc{Name} & \textsc{Description} & \textsc{Links} \\
\midrule
\TextCircle\VisionCircle\SpeechCircle & \textbf{AI Vulnerability Database} & An open-source, extensible knowledge base of AI failures. & \emojiblank\emojiblank\emojiblank\href{https://avidml.org/}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Llama 2 Responsible Use Guide} & Guidance for downstream developers on how to responsibly build with Llama 2. Includes details on how to report issues and instructions related to red-teaming and RLHF. & \emojiblank\emojiblank\emojiblank\href{https://ai.meta.com/llama/responsible-use-guide/}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{BigScience Ethical Charter} & Outlines BigScience's core values and how they promote them, which in turn guides use restrictions. & \emojiblank\emojiblank\emojiblank\href{https://bigscience.huggingface.co/blog/bigscience-ethical-charter}{\eweb} \\

\TextCircle\VisionCircle\SpeechCircle & \textbf{Model Monitoring in Practice Tutorial} & A tutorial given at FAccT and other venues describing how and why to monitor ML models. Includes a presentation on using transformer models to monitor for error detection. & \emojiblank\emojiblank\emojiblank\href{https://sites.google.com/view/model-monitoring-tutorial}{\eweb} \\
\TextCircle\VisionCircle\SpeechCircle & \textbf{Model Gating from Hugging Face} & A resource describing how to require user credentials for model access, which may be appropriate for models trained for topics such as hate speech. & \emojiblank\emojiblank\emojiblank\href{https://huggingface.co/docs/hub/models-gated}{\eweb} \\
\bottomrule
\end{tabular}
\end{table}


